MedHorizon: Towards Long-context Medical Video Understanding in the Wild

Medical multimodal large language models (MLLMs) have advanced image understanding and short-video analysis, but real clinical review often requires full-procedure video understanding. Unlike general long videos, medical procedures contain highly redundant anatomical views, while decisive evidence is temporally sparse, spatially subtle, and context dependent. Existing benchmarks often assume this evidence has already been localized through images, short clips, or pre-segmented videos, leaving the retrieval-before-reasoning problem under-tested. We introduce MedHorizon, an in-the-wild benchmark for long-context medical video understanding. MedHorizon preserves 759 hours of full-length clinical procedures and provides 1,253 evidence-grounded multiple-choice questionsthat jointly evaluate sparse evidence understanding and multi-hop clinical reasoning. Its evidence is extremely sparse, with only 0.166% evidence frames on average, requiring models to search noisy procedural streams before interpreting and aggregating findings. We evaluate representative general-domain, medical-domain, and long-video MLLMs. The best model reaches only 41.1% accuracy, showing that current systems remain far from robust full-procedure understanding. Further analysis yields four key findings: performance does not scale reliably with more frames, evidence retrieval and clinical interpretation remain primary bottlenecks; these bottlenecks are rooted in weak procedural reasoning and attention drift under redundancy, and generic sampling methods only partially balances local detail with global coverage. MedHorizon provides a rigorous testbed for MLLMs that retrieve sparse evidence and reason over complete clinical workflows.

==> MLVBench_NeurIPS2026_Overleaf/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract, introduction, benchmark construction, and experiments all make the same core claim: existing MLLMs remain weak when sparse evidence retrieval and multi-hop reasoning must be solved jointly in full-procedure medical video.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The conclusion explicitly states two limitations of the current benchmark: reliance on public-source video diversity and a multiple-choice protocol that cannot fully capture free-form clinical reporting.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present new theoretical results or formal proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sections 3 and 4 describe the source datasets, question construction pipeline, evaluation split, task taxonomy, model families, and frame-budget settings that support the main experimental claims.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The benchmark is built on public source videos, and the benchmark assets are paired with the evaluation protocol used in this paper so the reported results can be reproduced in anonymized form.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 4 specifies the benchmark size, task structure, model categories, and frame-budget settings used in the comparisons and analyses, while Section 3 defines how the benchmark itself is constructed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: We report deterministic benchmark accuracies on a fixed evaluation set, but we do not include repeated-run error bars or formal significance tests.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper reports model types and frame budgets, but it does not provide a full per-experiment accounting of hardware, memory, runtime, and total compute.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work uses public or previously released clinical video sources for benchmark construction and is intended for evaluation research rather than direct clinical deployment, which is consistent with the NeurIPS Code of Ethics to the best of our knowledge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The conclusion discusses both the positive value of more realistic clinical-video evaluation and the risk of over-interpreting benchmark performance as readiness for autonomous clinical deployment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper releases an evaluation benchmark rather than a high-risk generative model, and all underlying videos come from public or previously released sources, so this question is not central to the contribution.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The source datasets and prior assets are cited throughout Sections 2 and 3, but the paper does not enumerate the full license details for every existing asset in the main text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3 documents the new benchmark through source provenance, task definitions, question construction, and evaluation protocol, and the release materials are organized to mirror that structure.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve new crowdsourcing or prospective research with human subjects; it builds a benchmark from public or previously released datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve new crowdsourcing or prospective research with human subjects, so IRB-style approval is not applicable here.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3 states that GPT-5.4 is used in the benchmark construction pipeline for question rewriting and distractor refinement, making its role explicit where it affects the released benchmark formulation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> MLVBench_NeurIPS2026_Overleaf/conclusion.tex <==

\section{Conclusion}

We present \ours, an in-the-wild benchmark for long-context medical video understanding.  Representative general-domain, medical-domain, and retrieval-style MLLMs perform poorly, with the best model reaching only 41.1\% accuracy. Our analyses show that non-monotonic frame scaling, persistent bottlenecks in clinical evidence retrieval and interpretation, the weak procedural reasoning and attention drift, and the limited ability of generic sampling strategies. \ours remains limited by public-video diversity, annotation quality, and a multiple-choice protocol that cannot fully capture free-form clinical reporting, but offers a clear testbed for sparse evidence interpretation and full-procedure clinical reasoning in long-context medical videos.

==> MLVBench_NeurIPS2026_Overleaf/dataset.tex <==
% \setlength{\tabcolsep}{3pt}

% \section{Benchmark Construction}
% \label{sec:dataset}

% \subsection{Data Curation}

% \ours is built from 8 public medical video sources. The full corpus contains 340 videos, 759 decoded hours, a median duration of 83.2 minutes, and a maximum duration of 37.2 hours. It covers 7 organs and 4 scene types: surgical video, colonoscopy, capsule endoscopy, and ultrasound. This diversity matters. A model that only sees one procedure family can memorize local priors. Our benchmark instead asks the model to transfer across cardiac surgery, abdominal surgery, gynecologic surgery, neurosurgery, prostatectomy, gastrointestinal examination, and obstetric ultrasound.

% % \input{tables/source_datasets.tex}

% The benchmark also separates corpus coverage from evaluation depth. The 30-study ultrasound extension increases scene diversity and long-study coverage, but it only supports a study-level recognition task because the released annotations do not provide grounded timestamps. The main long-horizon benchmark therefore relies on the 7 richly annotated sources that support temporally anchored and compositional question construction.

% \begin{figure*}[ht]
%     \centering
%     \subfigure[Video Category.]{
%     \centering
%         \includegraphics[width=0.25\linewidth]{figures/category.pdf}
%         \label{fig:data_a}
%     }
%     \hfill
%         \subfigure[Video Duration Distribution]{
%         \includegraphics[width=0.4\linewidth]{figures/duration_distri.pdf}
%         \label{fig:data_b}
%     }
%     \hfill
%     \subfigure[QA density]{
%         \includegraphics[width=0.25\linewidth]{figures/qa_density.pdf}
%         \label{fig:data_c}
%     }
%     \hfill
% \end{figure*}

% \subsection{Construction Pipeline}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/all_demo.pdf}
%     \caption{Benchmark construction pipeline. Starting from source annotations, we generate task-specific questions, filter and rewrite them, and finalize a compact benchmark for visually grounded long-video evaluation.}
%     \label{fig:pipeline}
% \end{figure}

% The benchmark is not a direct dump of template-generated base questions. We start from source annotations and task templates that cover phase and step understanding, region and exam recognition, lesion characterization, instrument recognition, and procedure-level reasoning. We then filter noisy or temporally invalid items, balance answer distributions, rewrite questions into direct natural language with GPT-5.4, and strengthen distractors with nearby frames and clinically plausible alternatives. Finally, clinicians review rewritten and difficult samples. The result is a compact benchmark that requires models to use visual cues, temporal context, and clinical semantics together, rather than relying on text shortcuts or overly template-like single-step answering.

% The final benchmark contains 1,253 MCQs and is used throughout the paper for both model comparison and detailed diagnostic analyses.

% \subsection{Dataset Statistics}

% We summarize MLVBench by the dominant clinical skill each question requires. The benchmark covers phase and step understanding, region and exam recognition, lesion characterization, instrument recognition, counting and ranking, and procedure-level lesion summary. Most questions test fine-grained understanding over sparse evidence, while semantic reasoning tasks require multi-hop reasoning over observations scattered across the same procedure.

% % \input{tables/capability_taxonomy.tex}

% \begin{center}
% \begin{minipage}[t]{0.60\linewidth}
%     \centering
%     \vspace{0pt}
%     \includegraphics[width=\linewidth]{figures/MLVBench_pipeline.pdf}
%     \captionof{figure}{Benchmark construction pipeline. Starting from source annotations, we generate task-specific questions, filter and rewrite them, and finalize a compact benchmark for visually grounded long-video evaluation.}
%     \label{fig:pipeline}
% \end{minipage}\hfill
% \begin{minipage}[t]{0.34\linewidth}
%     \centering
%     \vspace{0pt}
%     \includegraphics[width=\linewidth]{figures/capability_taxonomy_radial.pdf}
%     \captionof{figure}{Task taxonomy of MLVBench. The benchmark spans both fine-grained understanding and semantic reasoning across diverse clinical skills.}
%     \label{fig:capability_taxonomy}
% \end{minipage}
% \end{center}


% This benchmark differs from recent medical video-language datasets in two ways. First, \ours keeps the full procedure whenever possible instead of trimming the task to short clips. Second, it mixes multiple clinical scenes rather than staying inside one specialty. \tabref{tab:recent_compare} therefore uses a compact property matrix instead of long textual summaries. It shows that recent datasets from 2024--2026 usually cover only surgery or only examination, often work on clips rather than full procedures, and rarely make long-context reasoning the core evaluation target. \ours is the only benchmark in this comparison that checks every property column.

% \input{tables/recent_compare.tex}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/pipeline.pdf}
    \caption{Benchmark construction pipeline.}
   \label{fig:pipeline}
\end{figure}


\begin{figure*}[ht]
    \centering
    \subfigure[Video Category.]{
    \centering
        \includegraphics[width=0.25\linewidth]{figures/category.pdf}
        \label{fig:data_a}
    }
    \hfill
        \subfigure[Video Duration Distribution]{
        \includegraphics[width=0.4\linewidth]{figures/duration_distri.pdf}
        \label{fig:data_b}
    }
    \hfill
    \subfigure[QA density]{
        \includegraphics[width=0.25\linewidth]{figures/qa_density.pdf}
        \label{fig:data_c}
    }
    \hfill
    \caption{Overview of the source corpus.}
    \label{fig:data_overview}
\end{figure*}

% \begin{center}
% \begin{minipage}[t]{0.63\linewidth}
%     \centering
% \includegraphics[width=\linewidth]{figures/pipeline.pdf}
%     \captionof{figure}{Benchmark construction pipeline.}
%     \label{fig:pipeline}
% \end{minipage}\hfill
% \begin{minipage}[t]{0.34\linewidth}
%     \centering

%     \includegraphics[width=\linewidth]{figures/capability_taxonomy.pdf}
%     \captionof{figure}{Task taxonomy.}
%     \label{fig:capability_taxonomy}
% \end{minipage}
% \end{center}


\setlength{\tabcolsep}{3pt}

\section{Benchmark Construction}
\label{sec:dataset}

\subsection{Data Curation}

\ours is built from 8 public medical video sources, totaling 340 videos and 759 decoded hours across 7 organs and 2 clinical scene types, including surgery, colonoscopy, capsule endoscopy, and ultrasound, as summarized in \figref{fig:data_overview}(a). This breadth prevents long-context medical video understanding from collapsing to a single procedure family or annotation style, and forces transfer across distinct visual appearances, workflows, and temporal rhythms, including cardiac and abdominal surgery, gastrointestinal examination, and obstetric ultrasound.

The source corpus is deliberately long-tailed in duration: \figref{fig:data_overview}(b) shows many videos last over one hour, with the longest study reaching 37.2 hours. This matters because realistic deployment retrieval bottlenecks come from searching full procedural streams, not pre-trimmed clips. As illustrated in \figref{fig:data_overview}(c), question density varies considerably across datasets, primarily driven by discrepancies in temporal granularity and clinical scope among released annotations. Consequently, we decouple corpus coverage from evaluation depth in our subsequent construction phase.




\subsection{Construction Pipeline}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/mlvbench_demo_0506_cropped.pdf}
    \caption{Representative video-question pairs across fine-grained understanding and semantic reasoning tasks in \ours.}
    \label{fig:all_demo}
\end{figure}

The benchmark is constructed through the evidence grounded pipeline in \figref{fig:pipeline}. Starting from diverse surgical and examination videos, we collect source annotations and task schemas covering phases,  anatomical regions, examination targets, lesion properties, instruments, and procedure level events. 

In the second step, each QA item is generated from explicit video evidence in expert annotations. The process retrieves evidence from the full video, including sparse key frames and temporally relevant segments, then builds candidate questions around the annotated event or finding. We filter noisy, ambiguous, or temporally inconsistent candidates, balance answer distributions, rewrite questions into direct natural language with GPT 5.4, and strengthen distractors using nearby temporal events and clinically plausible alternatives. This design gives every retained question a traceable visual basis and challenging distractors without unsupported claims. 

The final construction stage, human in the loop verification, uses human review as an audit layer. In each construction iteration, all items went through four checks: whether the video is usable for the intended task, whether the question and answer choices are well formed, whether the selected evidence truly supports the answer, and whether the final label is consistent with the original annotation. Items failing these checks are revised or removed, keeping the benchmark grounded in observable video content rather than post hoc textual assumptions. Detailed audit statistics, construction funnel counts, evidence export fields, and the oracle evidence protocol are provided in the appendix \ref{sec:supp_benchmark_card}.

% This evidence based construction gives \ours its central distinction. As shown in \figref{fig:all_demo}, the benchmark evaluates fine grained understanding and semantic reasoning over raw long videos. Fine grained tasks test localization of subtle visual cues, including phase transitions, anatomical regions, lesion appearance, instrument identity, and examination findings. Semantic reasoning tasks require connecting these cues across time, for example comparing repeated findings, binding observations to anatomical context, identifying a dominant maneuver, or aggregating multiple lesions into a procedure level judgment. The model is evaluated on the original long video rather than pre selected answer clips; relevant evidence may be sparse, temporally distant, and visually subtle. Thus, \ours moves beyond single label recognition and measures search, understanding, and reasoning over clinically meaningful video evidence.

\subsection{Dataset Statistics}

% We categorize \ours by the dominant clinical skill required for each question. As shown in \figref{fig:capability_taxonomy}, the benchmark spans both fine-grained understanding and semantic reasoning. The tasks evaluated are: Phase Recognition (PR), Step Discrimination (SD), Region Localization (RL), Bowel Preparation Quality (BPQ), Largest-Lesion Size (LLS), Lesion-Site Binding (Site), Histology Binding (Hist), Lesion-Size Binding (Size); Instrument Recognition (IR), Workload Ranking (WR), Ranked Step Retrieval (RSR), Count-Proportion Reasoning (CPR), and Lesion Analysis (LA). This heterogeneity prevents the benchmark from collapsing into a single pattern, balancing local discrimination under sparse evidence with cross-temporal integration across entire procedures.
% We categorize \ours by the dominant clinical skill required for each question. 
% As shown in \figref{fig:capability_taxonomy}, the benchmark spans both fine-grained understanding and semantic reasoning. 
% Specifically, PR recognizes procedural phases, SD distinguishes visually similar procedural steps, RL localizes anatomical regions, BPQ assesses bowel cleanliness and mucosal visibility, and LLS identifies the largest lesion and its size. 
% The binding tasks associate a lesion with its anatomical site (Site), histological label (Hist), or size attribute (Size). 
% Beyond these fine-grained understanding tasks, we further stratify semantic reasoning tasks by reasoning depth. 
% Instrument Recognition (IR) is a one-hop visual-semantic understanding task, where the model maps a localized instrument appearance to its category. 
% Workload Ranking (WR) and Ranked Step Retrieval (RSR) require two-hop reasoning: WR first estimates workload-relevant cues for candidate segments and then compares their relative burden, while RSR first identifies procedural steps across time and then retrieves the step satisfying a specified temporal rank. 
% Count-Proportion Reasoning (CPR) and Lesion Analysis (LA) require three-hop reasoning: CPR locates repeated events, estimates their proportions, and aggregates them over the full procedure, whereas LA retrieves lesion-relevant moments, binds them to appearance, location, and temporal context, and integrates these observations for lesion-centric decision making. 
% This heterogeneity prevents the benchmark from collapsing into a single pattern, balancing local discrimination under sparse evidence with cross-temporal integration across entire procedures.

\begin{wrapfigure}{r}{0.45\linewidth}
\vspace{-2em}
  \centering
  \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/capability_taxonomy.pdf}
  \caption{Capability taxonomy.}
  \label{fig:capability_taxonomy}

\end{wrapfigure}
\ours is distinguished by its emphasis on evidence-based reasoning over raw, long-form clinical videos. As illustrated in  \figref{fig:all_demo} and \figref{fig:capability_taxonomy}, we categorize the benchmark into two primary dimensions: fine-grained understanding and multi-hop semantic reasoning. This hierarchy requires models to move beyond single-label recognition toward searching and integrating clinically meaningful evidence that is often sparse, temporally distant, and visually subtle. 
\textbf{Fine-grained understanding} tasks focus on the localization and identification of localized visual cues. This includes procedural phase recognition (PR), step discrimination (SD), anatomical region localization (RL), and assessment of bowel preparation quality (BPQ). Furthermore, "binding" tasks (Site, Hist, Size) and largest-lesion identification (LLS) require models to associate specific lesions with their respective anatomical, histological, or morphological attributes. \textbf{Semantic reasoning} tasks are further stratified by reasoning depth to measure cross-temporal integration. At the foundational level, \textbf{one-hop visual-semantic} tasks, such as Instrument Recognition (IR), require the model to map localized appearances to functional categories. Moving toward higher complexity, \textbf{two-hop} comparative tasks, including Workload Ranking (WR) and Ranked Step Retrieval (RSR), demand that models first identify procedural cues or steps across the timeline and subsequently perform relative comparison or temporal ranking. The highest level of complexity is captured by \textbf{three-hop} aggregative tasks, such as Count-Proportion Reasoning (CPR) and Lesion Analysis (LA). These require a sophisticated pipeline of locating repeated events or lesion-relevant moments, binding them to multi-dimensional contexts spanning appearance, location, and time, and finally aggregating these disparate observations into a unified, procedure-level clinical judgment.

% This heterogeneity prevents \ours from collapsing into simple pattern matching, balancing local discrimination with the need for global synthesis across entire medical procedures.


Finally, \tabref{tab:recent_compare} situates \ours relative to recent medical video benchmarks. Existing resources often focus on either surgery or examination, rely on short clips or pre-selected segments, or flatten evaluation into atomic recognition. By contrast, \ours is the only benchmark in this comparison that jointly preserves full-procedure integrity, evaluates sparse evidence retrieval, and requires multi-hop reasoning across multiple clinical scenes.

\input{tables/recent_compare.tex}


==> MLVBench_NeurIPS2026_Overleaf/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate a diverse set of state-of-the-art MLLMs, grouped into closed-source MLLMs, general open-source video MLLMs, specialized long-video methods, and medical MLLMs. For closed-source models with native video input, we sample videos at 1 FPS and cap the input at 1,248 frames to ensure stable API inference on very long videos. For general open-source video MLLMs, models with native long-video support use 1 FPS decoding with the maximum-frame cap from their official implementations, while others use 64 uniformly sampled frames. For specialized long-video methods, we follow their official frame budgets and sampling strategies. For medical MLLMs, all evaluated models support native long-video inference, so we use 1 FPS decoding with their official maximum-frame caps. All models are evaluated with official settings and run on 8 A800.

Four research questions organize the analysis. \textbf{RQ1:} Does long-context medical video understanding follow a frame-scaling law as general domains? \textbf{RQ2:} What limits the performance of MLLMs in long-context medical video understanding? \textbf{RQ3:} What underlying mechanisms explain such bottlenecks? \textbf{RQ4:} Can generic sampling strategies address the unique challenges of long-context medical  videos understanding? 

% Four research questions organize the analysis. \textbf{RQ1:} Does long-context medical video understanding follow a frame-scaling law as in general long-video tasks? \textbf{RQ2:} What limits the performance of MLLMs in long-context medical video understanding? \textbf{RQ3:} What mechanisms explain the failure mode? \textbf{RQ4:} Can general long-video sampling strategies solve the long-context medical video problem? 

  
  % Together, these RQs map to two core benchmark axes: evidence localization in raw long videos and clinical reasoning over subtle, dispersed observations.


% \subsection{Overall Performance}

% \input{tables/main_results.tex}

% Table~\ref{tab:main_results} shows that long-context medical video understanding remains far from solved. The strongest model, Gemini-3.1-Pro-Preview, reaches 41.1\% overall, while most open and medical models cluster in the mid-20s. This gap is important: even large multimodal models that perform strongly on short-form understanding do not yet translate that competence into reliable full-procedure reasoning.

% The per-task pattern is more revealing than the overall average. Tasks with stronger global regularities, such as BPQ, are relatively easier, whereas Hist, LLS, and CPR remain weak across nearly all models. Taken together, the table shows that the central bottleneck is not generic language generation alone; it is robust use of long visual context for both evidence localization and cross-temporal reasoning.

\subsection{Overall Performance}

\input{tables/main_results.tex}

% Table~\ref{tab:main_results} demonstrates that long medical video understanding remains largely unsolved. The leading model, Gemini-3.1-Pro-Preview, achieves only 41.1\% accuracy, while most open-source and medical MLLMs hover around 25\%. This gap is significant as evaluation occurs under full-procedure contexts, requiring models to search redundant streams for sparse evidence and apply it to clinical judgment.

% Per-task results highlight this bottleneck more clearly. Tasks leveraging procedural regularities or salient cues, such as BPQ, RL, IR, and WR, show higher performance. Conversely, lesion-centric tasks like LLS, Site, Hist, and Size are more unstable, requiring models to locate subtle findings and bind them to anatomical or clinical attributes. Semantic-reasoning tasks further expose limitations; while RSR suggests procedural order provides a usable cue, CPR and LA remain difficult as they necessitate counting and aggregating distributed observations.

% These results underscore the core finding of \ours: the primary obstacle is the coupling between sparse evidence localization and cross-temporal reasoning. Although current MLLMs exploit coarse global cues or isolated salient frames, they struggle when answers depend on subtle evidence, attribute binding, or aggregating distant events. This suggests longer context windows are insufficient without mechanisms to selectively retrieve weak evidence and maintain structured clinical context throughout the procedure.

Table~\ref{tab:main_results} shows that long medical video understanding remains substantially unsolved. The strongest model, Gemini-3.1-Pro-Preview, reaches only 41.1\% overall accuracy, while most open-source and medical MLLMs remain around the mid-20s. This gap is notable because evaluation is conducted under full-procedure video context. Models must therefore not only recognize medical visual content, but also search long redundant streams for sparse evidence and use it for clinical judgment. The per-task results reveal this bottleneck more clearly than the overall score. Tasks that can benefit from broader procedural regularities or salient visual cues, such as BPQ, RL, IR, and WR, show relatively higher peaks. In contrast, lesion-centric tasks such as LLS, Site, Hist, and Size are more unstable across models, since they require locating subtle local findings and binding them to anatomical sites or clinical attributes. Semantic-reasoning tasks further expose the weakness of current long-video reasoning. RSR is often stronger, suggesting that procedural order provides a usable cue, whereas CPR and LA remain difficult because they require counting, comparing, and aggregating distributed observations across the same procedure.

These results underscore the core finding of \ours: the primary obstacle is the coupling between sparse evidence localization and cross-temporal reasoning. Although current MLLMs exploit coarse global cues or isolated salient frames, they struggle when answers depend on subtle evidence, attribute binding, or aggregating distant events. This suggests longer context windows are insufficient without mechanisms to selectively retrieve weak evidence and maintain structured clinical context throughout the procedure.

\begin{wrapfigure}{r}{0.45\linewidth}

  \centering
  \includegraphics[width=\linewidth]{figures/frame.pdf}
  \caption{Frame-scaling performance under different sampled-frame budgets.}
  \label{fig:frame_scaling}

\end{wrapfigure}

\subsection{RQ1: Frame Scaling Is Unreliable in Medical Long Videos.}

% Figure~\ref{fig:frame_scaling} studies whether increasing the number of sampled frames improves long-context medical video understanding. We vary the frame budget from 4 to 512 on the same set of questions. Unlike the simple expectation that more frames should provide better coverage, performance does not improve monotonically. Qwen3-VL-8B remains relatively stable and reaches its best accuracy at 256 frames, but drops when the input increases to 512 frames. Lingshu-7B shows a sharper failure pattern: it peaks at 32 frames with 26.3\% accuracy, then degrades consistently and falls to 17.3\% at 512 frames.

% This result suggests that medical long videos do not obey a straightforward frame-scaling law. Additional frames can increase the chance of covering sparse evidence, but they also introduce highly redundant anatomy, irrelevant procedural segments, and visually similar distractors. Without effective evidence selection, larger context may dilute rather than strengthen the useful signal. Thus, simply scaling the number of frames is insufficient for long-context medical video understanding.



Figure~\ref{fig:frame_scaling} tests whether medical long-video accuracy improves as more frames are sampled from the same videos. The main observation is the absence of a consistent positive slope. Qwen3-VL-8B is comparatively robust, but its curve mostly oscillates within a narrow band: it improves again at 128--256 frames and then drops at 512 frames. Lingshu-7B benefits only from a small-to-moderate budget, reaching its best result at 32 frames before steadily declining as the input becomes longer. MedGRPO shows the clearest context-dilution effect: adding frames does not recover more evidence, but instead drives accuracy downward from 4 to 512. 

These different curve shapes indicate that frame count is not the controlling variable for reliable medical video understanding. More frames can improve the chance of including sparse clinical evidence, but they also add near-duplicate anatomy, low-information procedural segments, and visually similar distractors. Current models do not consistently convert the extra visual context into better evidence use: Qwen3-VL-8B tolerates longer inputs without a clear gain, while the medical-domain models degrade once redundant context dominates the useful signal. Thus, the bottleneck is not merely insufficient temporal coverage, but the lack of evidence-aware selection and compression. Long-context medical MLLMs need mechanisms that retrieve subtle decisive frames and suppress redundant context, rather than simply increasing the sampled-frame budget.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/E7.pdf}
%     \caption{ breakdown of various models on \ours under different input settings. The results highlight the severe retrieval bottleneck and the absence of language-driven shortcuts.}
%     \label{fig:e7}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/E7.pdf}
    \caption{Diagnostic breakdown under four input settings: random guessing, text-only questions, uniformly sampled full-video frames, and oracle GT-images. The comparison separates language shortcuts, temporal evidence retrieval, and post-retrieval evidence interpretation.}
    \label{fig:e7}
\end{figure}

\subsection{RQ2: Evidence Retrieval and Interpretation Remain Bottlenecks.}

% Figure~\ref{fig:e7} directly evaluates the understanding bottleneck. The Text-only baseline (Qwen3-VL-8B) aligns with or falls below the Random baseline of 25\%, indicating that \ours suppresses superficial language priors and forces models to rely on visual evidence. However, a large gap remains between Uniform sampling and GT-images. This gap shows that temporal evidence localization is a major failure mode: when decisive evidence occupies only a tiny fraction of the full procedure, standard sampling often misses the relevant moments entirely.

% The oracle GT-images setting further shows that temporal retrieval is not the only challenge. Even when models are given evidence frames, their performance remains modest and rarely exceeds 40\%. This means that models still struggle to interpret the retrieved evidence spatially and clinically. They must identify subtle local findings, distinguish similar anatomical appearances, estimate lesion attributes, and bind them to sites or phases before reasoning. For example, MedGRPO collapses to 13.6\% on Semantic tasks under uniform sampling, far below random, showing that reasoning ability becomes ineffective when evidence retrieval fails. Therefore, current MLLMs lack both reliable temporal localization and fine-grained visual evidence understanding for long medical videos.

% Figure~\ref{fig:e7} diagnoses evidence use with four input settings: \textit{Random} is the 25\% chance baseline, \textit{Text} removes all visual input, \textit{Uniform} uses sampled frames from the full procedure, and \textit{GT-images} provides human-verified evidence frames as an oracle. This design separates language shortcuts, temporal evidence retrieval, and post-retrieval visual interpretation. The results show that \ours is not mainly solved by language priors. Text-only accuracy stays close to random, while uniform video input brings limited and unstable gains. For example, MedGRPO drops to 13.6\% on Semantic tasks under uniform sampling, suggesting that irrelevant but plausible frames can actively mislead reasoning when sparse evidence is missed.

% The Uniform-to-GT-images gap reveals the retrieval bottleneck, especially for Semantic reasoning: MedGRPO improves from 13.6\% to 33.9\%, and Lingshu-7B from 22.9\% to 38.0\%. Yet even with oracle evidence, all models remain below 40\%, showing that retrieval is only the first failure mode. Models must still identify subtle local findings, distinguish similar anatomical appearances, and bind observations to sites, phases, or repeated events. Thus, RQ2 exposes a two-stage bottleneck: current MLLMs need both evidence-aware temporal retrieval and clinically grounded visual verification.


Figure~\ref{fig:e7} diagnoses evidence utilization across four settings: \textit{Random} (25\% baseline), \textit{Text} (no visual input), \textit{Uniform} (full-procedure sampling), and \textit{GT-images} (human-verified oracle frames). This separates language shortcuts, temporal retrieval, and visual interpretation. Results show \ours is not solvable by language priors alone; text-only accuracy mirrors the random baseline, while uniform video input yields limited, unstable gains. Notably, MedGRPO drops to 13.6\% on Semantic tasks under uniform sampling, suggesting irrelevant frames can mislead understanding when sparse evidence is missed. The Uniform-to-GT-images gap highlights a retrieval bottleneck, particularly for Semantic reasoning: MedGRPO improves from 13.6\% to 33.9\%, and Lingshu-7B from 22.9\% to 38.0\%. However, even with oracle evidence, all models remain below 40\%, proving retrieval is only the initial failure mode. Models must still identify subtle findings, distinguish similar anatomy, and bind observations to phases or events. Thus, RQ2 exposes a dual bottleneck: MLLMs require both evidence-aware temporal retrieval and clinically grounded visual verification.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/e1.pdf}
    \caption{Disrupting event order consistently hurts performance. That there is only a slight performance decrease underscores the models' inability to effectively exploit temporal information.}
    \label{fig:e1}
\end{figure}

\begin{figure}[t]
    \centering

        \includegraphics[width=0.9\linewidth]{figures/attn.pdf}
    \caption{Attention distribution and similarity in frame and patch-level.}
    % \caption{Attention remains broadly spread rather than collapsing onto a few decisive moments, despite the high visual redundancy of the video stream.}
    \label{fig:e6}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/e2.pdf}
    \caption{Frame-change sampling helps short-window tasks, but uniform sampling remains the most stable overall strategy. And other generic sampling methods also have limited improvement.}
    \label{fig:e2}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/e3_large.pdf}
%     \caption{Changing how the same frame budget is allocated shifts wins and losses across tasks while leaving overall accuracy nearly unchanged.}
%     \label{fig:e3}
% \end{figure}

\subsection{RQ3: Weak Procedural Reasoning and Attention Drift under Redundancy.}

% % The frame-level diagnostics show that medical long videos behave differently from the common general-video assumption that redundant frames can be safely compressed into a few salient moments. Figure~\ref{fig:e1} first tests whether models use event order. When the sampled frames are reversed or shuffled, Qwen3-VL-8B drops from 26.5\% to about 24.2--24.5\%, with clearer losses on workflow-sensitive tasks such as PR and IR. This indicates that temporal order matters, but the modest drop also suggests that current models use procedural chronology only weakly.
% % % 应该说明：左边对应temporal，右边对应spatial。frame-level的attention线性增加，这说明每一帧的attn都一样，并且qwen和lingshu两个相似度都维持很高 90%，而MedGRPO略低一些，说明temporal 数据训练可以加强encoder对于不同帧的分辨力。而右边spatial同样说明attn没用，而lingshu这种大规模domain knowledge pretrain过的，
% % Figure~\ref{fig:e6} reveals a complementary attention pattern that depart from general long videos \cite{cheng2025scaling} . Attention does not collapse onto a small number of decisive frames. Qwen3-VL-8B and Lingshu-7B still require 76.7\% and 85.6\% of temporal units, respectively, to accumulate 90\% of frame-level attention. And MedGRPO as a medical video MLLM, its behavior is quite similar with Qwen3-VL. In other words, the videos are visually redundant, but the models cannot identify which similar-looking moments carry clinical evidence.

% % This behavior highlights a key difference between medical and general long-video understanding. In medical videos, redundancy is deceptive: many frames look similar, yet only a few contain subtle clinically decisive findings. As a result, attention spreads across broad temporal regions instead of concentrating on the useful evidence. This explains why longer context windows and generic key-frame compression are both insufficient without medical evidence-aware selection.

% Figure~\ref{fig:e1} shows that current models use temporal order only weakly. Reversing, block-shuffling, or locally shuffling frames reduces Qwen3-VL-8B from 26.5\% to 24.2--24.5\% overall, with larger losses on workflow- or context-sensitive tasks such as PR, IR, QA, LLS, and CPR. This confirms that chronology matters, but the small overall drop suggests that the model mainly captures coarse temporal cues rather than robust procedural structure.
% % Then we test whether medical long videos follow the redundancy patterns observed in general long-video understanding. Following ViLAMP~\cite{vilamp}, we diagnose query-induced attention at frame and patch levels. For each video-question pair, we sample 128 frames, aggregate query-to-visual attention into frame scores, and plot cumulative attention after ranking frames by attention. For patch-level analysis, we use the top 32 attended frames as keyframes and compare patches in the remaining 96 frames with their corresponding patches in the nearest preceding keyframe. Thus, the left half of Figure~\ref{fig:e6} measures temporal redundancy, and the right half measures spatial redundancy.
% Then we test whether medical long videos follow the redundancy patterns of general video understanding. Following ViLAMP~\cite{vilamp}, we diagnose query-induced attention at frame and patch levels. We sample 128 frames per pair, aggregate query-to-visual attention into frame scores, and plot cumulative attention by rank. For patch-level analysis, the top 32 attended frames serve as keyframes to compare patches in the remaining 96 frames with their preceding keyframe counterparts. Thus, Figure~\ref{fig:e6} measures temporal (left) and spatial (right) redundancy. It reveals that medical videos break the intuition that attention collapses onto few salient frames. Cumulative curves increase smoothly; Qwen3-VL-8B and Lingshu-7B require 76.7\% and 85.6\% of units to reach 90\% attention, with MedGRPO similarly diffuse. Qwen3-VL-8B and Lingshu-7B maintain high frame similarity, while MedGRPO is slightly lower, suggesting medical training may improve discriminability but not selective attention. Spatial panels show high-attention patches remain highly similar to keyframes, especially for Lingshu-7B. Thus, medical redundancy is deceptive: many frames look alike, but answers depend on subtle outliers that current attention fails to isolate.

% % Figure~\ref{fig:e6} further shows that medical videos break the general-video intuition that attention should collapse onto a few salient frames. The frame-level cumulative curves increase smoothly, so Qwen3-VL-8B and Lingshu-7B still require 76.7\% and 85.6\% of temporal units to accumulate 90\% attention, and MedGRPO remains similarly diffuse. Meanwhile, Qwen3-VL-8B and Lingshu-7B maintain very high frame similarity around 0.90, while MedGRPO is slightly lower, suggesting that medical-video training may improve frame discriminability but not evidence-selective attention. The patch-level panels show the same issue spatially: high-attention patches remain highly similar to keyframe patches, especially for Lingshu-7B. Thus, medical redundancy is deceptive---many frames and patches look alike, but the answer often depends on a subtle outlier that current attention mechanisms fail to isolate.

% We use two complementary diagnostics to test whether medical long videos follow general long-video intuitions. 


% We analyze the mechanisms behind these bottlenecks by diagnosing how models handle temporal structure and visual attention distribution. Figure~\ref{fig:e1} perturbs frame order to measure whether models use procedural chronology, while Figure~\ref{fig:e6} follows ViLAMP~\cite{vilamp} to diagnose whether attention concentrates on informative frame- and patch-level evidence. For each video-question pair, we sample 128 frames, aggregate query-to-visual attention into frame scores, and plot cumulative attention after ranking frames by attention. For patch-level analysis, we use the top 32 attended frames as keyframes and compare patches in the remaining 96 frames with their corresponding patches in the nearest preceding keyframe. Thus, the left half of Figure~\ref{fig:e6} measures temporal redundancy, and the right half measures spatial redundancy. Figure~\ref{fig:e1} shows that current models use temporal order only weakly. Reversing, block-shuffling, or locally shuffling frames reduces Qwen3-VL-8B from 26.5\% to 24.2--24.5\% overall, with larger losses on workflow- or context-sensitive tasks such as PR, IR, QA, LLS, and CPR. This confirms that chronology matters, but the small overall drop suggests that the model mainly captures coarse temporal cues rather than robust procedural structure. Figure~\ref{fig:e6} further shows that medical videos break the general-video intuition that attention should collapse onto a few salient frames. The frame-level cumulative curves increase smoothly, so Qwen3-VL and Lingshu still require 76.7\% and 85.6\% of temporal units to accumulate 90\% attention, and MedGRPO remains similarly diffuse. Meanwhile, Qwen3-VL-8B and Lingshu-7B maintain very high frame similarity around 0.90, while MedGRPO is slightly lower, suggesting that medical-video training may improve frame discriminability but not evidence-selective attention. The patch-level panels show the same issue spatially: high-attention patches remain highly similar to keyframe patches, especially for Lingshu-7B. Thus, medical redundancy is deceptive: many frames and patches look alike, but the answer often depends on a subtle outlier that current attention mechanisms fail to isolate.


  We analyze the mechanisms behind these bottlenecks by diagnosing how models handle temporal
  structure and visual attention distribution. Figure~\ref{fig:e1} perturbs frame order to measure
  whether models use procedural chronology, while Figure~\ref{fig:e6} follows ViLAMP~\cite{vilamp} to
  diagnose whether attention concentrates on informative frame- and patch-level evidence. For each
  video-question pair, we sample 128 frames, aggregate query-to-visual attention into frame scores,
  and plot cumulative attention after ranking frames by attention. For patch-level analysis, we use
  the top 32 attended frames as keyframes and compare patches in the remaining 96 frames with their
  corresponding patches in the nearest preceding keyframe. Thus, the left half of Figure~\ref{fig:e6}
  measures temporal redundancy, and the right half measures spatial redundancy. Figure~\ref{fig:e1} shows that current models use temporal order only weakly. Reversing, block-
  shuffling, or locally shuffling frames reduces Qwen3-VL-8B from 26.5\% to 24.2--24.5\% overall,
  with larger losses on workflow- or context-sensitive tasks such as PR, IR, QA, LLS, and CPR. This
  confirms that chronology matters, but the small overall drop suggests that the model mainly
  captures coarse temporal cues rather than robust procedural structure. Figure~\ref{fig:e6} further shows that medical videos break the general-video intuition that
  attention should collapse onto a few salient frames. The frame-level cumulative curves increase
  smoothly, so Qwen3-VL and Lingshu still require 76.7\% and 85.6\% of temporal units to accumulate
  90\% attention, and MedGRPO remains similarly diffuse. Meanwhile, Qwen3-VL-8B and Lingshu-7B
  maintain very high frame similarity around 0.90, while MedGRPO is slightly lower, suggesting that
  medical-video training may improve frame discriminability but not evidence-selective attention. The
  patch-level panels show the same issue spatially: high-attention patches remain highly similar to
  keyframe patches, especially for Lingshu-7B. We refer to this phenomenon as \textit{attention
  drift}: under strong spatiotemporal redundancy, model attention drifts toward visually repetitive
  but clinically non-decisive frames and patches, rather than reliably concentrating on sparse
  answer-relevant evidence. Thus, medical redundancy is deceptive: many frames and patches look
  alike, but the answer often depends on a subtle outlier that current attention patterns fail to
  isolate.



\subsection{RQ4: Generic Sampling Trades Local Detail for Global Coverage.}

% Figure~\ref{fig:e2} tests whether sampling can mitigate the long-context medical video problem. Uniform sampling is most stable by preserving broad procedural coverage, but remains evidence-agnostic and may miss short, sparse findings. Change-focused samplers improve short-window tasks, including SD, RL, Hist, and Size, yet lose coverage on workflow-sensitive tasks such as PR. Thus, visually dynamic frames are not necessarily clinically decisive. And Table \ref{tab:main_results} also shows that specialized long-video sampling is promising but limited. With 128 frames, AKS, ViLAMP, and WFS-SB achieve 27.3\%, 27.0\%, and 28.1\% overall accuracy, respectively, outperforming several general open-source video MLLMs under fixed or native budgets. Gains concentrate on local evidence tasks: WFS-SB reaches 32.8\% on Site, the best among open-source models, and improves over Qwen3-VL-8B on Size and IR. This matches their designs: ViLAMP preserves selected keyframes with higher fidelity while compressing non-keyframes and WFS-SB uses semantic-boundary-aware selection to retain structured temporal context.
Figure~\ref{fig:e2} evaluates whether sampling mitigates long-video challenges. Uniform sampling remains stable by preserving procedural coverage but is evidence-agnostic, often missing sparse findings. Conversely, change-focused samplers improve short-window tasks like RL and Size but hinder workflow-sensitive tasks (e.g., PR), showing that visual dynamism does not guarantee clinical relevance. Table~\ref{tab:main_results} confirms specialized sampling is promising: with 128 frames, AKS, ViLAMP, and WFS-SB achieve 27.3\%, 27.0\%, and 28.1\% accuracy, outperforming general MLLMs. Gains are localized; notably, WFS-SB reaches 32.8\% on Site. This reflects their designs: ViLAMP prioritizes keyframe fidelity via compression, while WFS-SB employs semantic-boundary selection to retain structured temporal context. These improvements remain modest and task-dependent. The methods still underperform on tasks requiring global procedural continuity or multi-step aggregation, such as WR and RSR, where aggressive keyframe selection may discard temporal context for reasoning. Sampling can reduce redundancy and recover some sparse evidence, but cannot solve long medical video understanding alone. Future methods need clinically evidence-aware sampling that preserves global procedural structure, retrieves weak local findings, and verifies anatomical and temporal context before reasoning.

% Figures~\ref{fig:e2} and~\ref{fig:e3} examine whether sampling can solve the long-context medical video problem. Uniform sampling remains the most stable overall strategy because it preserves broad procedural coverage. However, it is evidence-agnostic and can miss short, sparse findings. Change-focused samplers help some short-window tasks, including SD, RL, Hist, and Size, but they lose coverage on broader workflow-sensitive tasks such as PR. Thus, selecting visually dynamic frames is not equivalent to selecting clinically useful evidence.

% The local-global allocation study in Figure~\ref{fig:e3} shows the same trade-off from another angle. Reallocating the same frame budget toward denser local views helps tasks such as BPQ, Hist, and some CPR questions, but hurts IR and other tasks that depend on global procedural continuity. The overall scores remain nearly tied, suggesting that sampling changes redistribute errors rather than remove the core bottleneck.

% These findings answer RQ4 in a limited but important way. General downsampling strategies can partially help by providing either stable coverage or denser local evidence, but no fixed sampling rule solves the benchmark. Long medical video understanding requires an adaptive strategy that preserves global procedural structure while selectively zooming into weak evidence. Future models need clinically aware retrieval, temporal indexing, and local evidence verification rather than uniform frame scaling alone.


























% \subsection{Evidence Grounding: Sparse Retrieval as the Primary Bottleneck}
% The heavy dependence on precise visual evidence is the defining characteristic of \ours. As shown in Fig.~\ref{fig:e7}, the ``Text-only'' baseline aligns with or falls below the ``Random'' baseline of 25\%, confirming that \ours effectively suppresses language priors and forces models to rely on visual grounding. However, a massive performance gap exists between ``Uniform'' sampling and ``GT-images''. For instance, in MedGRPO (Fig.~\ref{fig:e7}c), uniform sampling results in a performance collapse in Semantic tasks to 13.6\%, which is far below random. This indicates that when decisive evidence is as sparse as 0.1\%, standard uniform sampling fails to capture the sparse evidence and renders the model's reasoning capabilities useless.

% Even when provided with GT-images, the performance of state-of-the-art models remains modest and rarely exceeds 40\% accuracy. This limited upper bound suggests that sparse retrieval is only the first hurdle; even with correct evidence, models still struggle with fine-grained visual characterization and complex semantic aggregation across distant moments. As illustrated in Fig.~\ref{fig:e7}, the jump from uniform to GT-informed performance is substantial yet far from diagnostic reliability. These findings reveal that long-context medical video understanding requires a dual breakthrough: highly efficient temporal indexing to overcome extreme sparsity, and specialized clinical reasoning depth to accurately interpret retrieved evidence.

% \subsection{Event Order Helps, But Models Use It Weakly}

% When we preserve the frame budget but disrupt event order, performance consistently drops. Reversing or shuffling the sampled frames reduces Qwen3-VL-8B from 26.5\% to about 24.2--24.5\%, with the clearest losses on workflow-sensitive tasks such as phase recognition (PR) and instrument recognition (IR). Thus, temporal order does matter, but the gain is modest.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.94\linewidth]{figures/E1.pdf}
%     \caption{Disrupting event order consistently hurts performance, especially on workflow-sensitive tasks.}
%     \label{fig:e1}
% \end{figure}

% This result is significant because it isolates one of the core requirements of procedural medicine: recognizing \emph{what} happened is not enough without knowing \emph{when} it happened. If current models had no temporal representation, order corruption would not matter; if they had robust long-range temporal reasoning, the penalty would be much larger. \figref{fig:e1} therefore suggests an intermediate regime in which models extract some chronological signal but still fail to internalize the full procedural structure needed for dependable review.



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.94\linewidth]{figures/e2.pdf}
%     \caption{Frame-change-focused sampling helps short-window tasks, but uniform sampling remains the most stable overall strategy.}
%     \label{fig:e2}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/e3_ladar.pdf}
%     \caption{Changing how the same frame budget is allocated shifts wins and losses across tasks while leaving overall accuracy nearly unchanged.}
%     \label{fig:e3}
% \end{figure}

% \subsection{Sparse Sampling Helps Some Tasks, Not the Benchmark}

% Changing the sampling strategy reveals a clear trade-off. Uniform sampling remains the most stable choice overall. Samplers that focus on frame changes help a narrow set of tasks with short evidence windows, especially step discrimination (SD), region localization (RL), lesion histology (Hist), and lesion size (Size), but they lose coverage on broader tasks such as PR that depend on the continuity of the procedure.


% The implication is that the benchmark is not merely an event-spotting problem. Some questions reward local, change-focused evidence, but others require stable procedural coverage, so any sampler that aggressively optimizes one side tends to hurt the other. \figref{fig:e2} therefore shows why sparse retrieval in medical video is fundamentally different from selecting a few ``interesting'' frames in natural video: clinically useful evidence may be sparse, but the surrounding procedural context still matters for interpretation.



% \subsection{Effect of Different Numbers of Frames}
%   Figure~\ref{fig:frame_scaling} presents a frame-scaling analysis on our medical long-video
%   benchmark, where we vary the number of sampled frames from 4 to 512 while evaluating on the
%   same set of questions. The results show that increasing visual context does not lead to
%   monotonic performance gains. Qwen3-8B remains relatively robust across different frame
%   budgets, with accuracy fluctuating within a narrow range and reaching its best performance
%   at 256 frames, but its accuracy drops when further increasing the input to 512 frames. In
%   contrast, Lingshu-7B benefits only from a moderate number of frames, peaking at 32 frames
%   before degrading consistently as more frames are added, falling from 26.3\% at 32 frames to
%   17.3\% at 512 frames. This trend highlights a key challenge in medical long-video
%   understanding: clinically relevant evidence is often sparse and temporally localized, while
%   additional frames introduce substantial redundancy, visually similar contexts, and
%   irrelevant procedural segments. Therefore, strong performance on this benchmark requires
%   not only larger visual context, but also effective evidence selection, temporal
%   aggregation, and robustness to long-context visual noise.
% \subsection{Local Detail and Global Coverage Still Compete}

% Reallocating the same frame budget between broad coverage and dense local views does not solve the benchmark. The overall scores stay nearly tied, yet task preferences move sharply. Denser local allocation helps quality assessment, lesion histology (Hist), and some count/proportion reasoning (CPR) questions, but hurts instrument recognition (IR) and other workflow-sensitive tasks.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/e3_ladar.pdf}
%     \caption{Changing how the same frame budget is allocated shifts wins and losses across tasks while leaving overall accuracy nearly unchanged.}
%     \label{fig:e3}
% \end{figure}

% This behavior is important because it separates a sampling problem from a representation problem. If frame budget allocation alone were the main obstacle, one allocation strategy would dominate. Instead, \figref{fig:e3} shows that current models still trade off local detail against global coverage, so changing the sampling pattern mostly redistributes errors rather than resolving them.

% \subsection{Attention Spreads Across Too Many Frames}

% The last analysis asks whether attention naturally collapses onto a few decisive medical frames just like general long videos. It does not. Across both Qwen3-VL-8B and the medical-domain LingShu-7B, random-pair frame similarity remains high, around 0.90, yet the models still need 76.7\% and 85.6\% of temporal units, respectively, to accumulate 90\% of frame-level attention. In other words, the videos are redundant, but attention still fails to concentrate on the clinically decisive moments.

% \begin{figure}[t]
%     \centering

%         \includegraphics[width=\linewidth]{figures/attn.pdf}

%     \caption{Attention remains broadly spread rather than collapsing onto a few decisive moments, despite the high visual redundancy of the video stream.}
%     \label{fig:e6}
% \end{figure}

% This result sharpens the central claim of the paper. The difficulty is not merely that medical videos are long or redundant; it is that decisive evidence is sparse and often ambiguous even among highly similar frames. When the model cannot distinguish which of those similar-looking moments actually matter, attention diffuses across a wide temporal window instead of collapsing onto the useful evidence. The same pattern appears in both general-domain and medical-domain models, suggesting that simply providing more frames is unlikely to solve the problem without better evidence localization and temporal selection.


==> MLVBench_NeurIPS2026_Overleaf/introduction.tex <==



% \section{Introduction}

% Long medical videos are central to ensuring diagnostic integrity, surgical precision, and clinical review. In colonoscopy, the clinical quality depends on the continuity of mucosal inspection and the quality of bowel preparation throughout the entire withdrawal phase~\cite{asge2024quality, corley2014adr}. Similarly, obstetric ultrasound requires the verification of standard views and sufficient anatomical coverage across an entire study rather than relying on a single representative snapshot~\cite{salomon2022isoug}. Surgical review also demands the ability to track phases and reason over critical events that are often separated by significant temporal gaps~\cite{demir2023workflow}. While Multimodal Large Language Models (MLLMs) are increasingly applied to these procedural settings, robust evaluation methodologies still lag behind the requirements of actual clinical use cases.

% The advancement of this field is primarily hindered by two gaps in existing evaluation paradigms. First, existing benchmarks fail to address the extreme temporal sparsity of realistic clinical video streams. In practice, diagnostically decisive evidences are buried within hours of routine and redundant footage, yet most benchmarks rely on pre-segmented clips that bypass the retrieval bottleneck. Second, existing resources under-test non-atomic clinical reasoning. Real clinical queries often require models to connect temporally dispersed observations into a holistic judgment, whereas current benchmarks frequently reduce evaluation to clip-level recognition or single-hop question answering~\cite{he2024pitvqa, li2024ophnet, thapa2025openbiomedvid, qian2026sureon}. As a result, they can overestimate performance in realistic full-context settings.

% To address these limitations, we introduce \ours, a comprehensive benchmark designed to capture the complex cognitive demands of long-context medical video understanding. Moving beyond the conventional expansion of video duration, the design philosophy of \ours centers on the synergistic interplay between fine-grained perceptual localization and high-level semantic reasoning. Leveraging a massive repository of 759 hours of raw, unedited clinical procedures and 1,253 expertly verified questions, \ours compels models to transcend local visual shortcuts and instead engage with the longitudinal clinical workflow.

% The key feature of \ours lies in its dual-layered design that reflects the in-the-wild nature of both data and queries. On the data dimension, \ours preserves the full procedural record rather than pre-selecting answer-bearing clips. This design creates an extreme retrieval bottleneck: compared with existing long-video benchmarks, \ours contains only 1.7 evidence frames per 1,000 video frames on average, and the mean question-level evidence ratio is 0.166\%, with 67.5\% of questions at or below 0.1\%, as shown in \figref{fig:main_teaser}(a--b). On the query dimension, \ours moves beyond atomic recognition to non-atomic clinical reasoning. \figref{fig:main_teaser}(c) makes the joint contrast explicit: in-the-wild data replace pre-cut short clips with raw long procedural videos, while in-the-wild queries replace atomic clip-level prompts with multi-hop clinical questions. For example, answering a lesion-distribution query requires retrieving sparse lesion frames, establishing the anatomical site corresponding to each lesion, and aggregating evidence across distant temporal windows before choosing the final answer. This formulation demands a form of procedural intelligence that more faithfully matches expert clinical review in real-world environments.

% % \begin{figure}[t]
% %     \centering
% %     \subfigure[]{
% %         \includegraphics[width=0.45\linewidth]{figures/1a.pdf}
% %     }
% %     \hfill
% %     \subfigure[]{
% %         \includegraphics[width=0.45\linewidth]{figures/1b.pdf}
% %     }
% %     \caption{Two properties make \ours challenging. (a) Useful frames are extremely sparse: the frames needed to answer a question occupy only 0.166\% of the source video on average, with several task groups far below that level. (b) \ours also goes beyond traditional single-hop clip QA by including semantic-reasoning questions that require whole-procedure aggregation and temporal comparison before a final answer can be chosen.}
% %     \label{fig:sparsity}
% % \end{figure}

% \begin{figure}[t]
%     \centering
%     % 使用 [t] 确保顶部对齐
%     \begin{minipage}[t]{0.4\linewidth}
%         \vspace{0pt} % 关键补丁：强制 minipage 的 anchor 在最顶端
%         \centering
%         \subfigure[]{
%             \includegraphics[width=\linewidth]{figures/1a.pdf}
%             \label{fig:sparsity_a}
%         }
        
%         % \vspace{1.5mm} % 调整 A 和 B 之间的垂直间距
        
%         \subfigure[]{
%             \includegraphics[width=0.85\linewidth]{figures/1b.pdf}
%             \label{fig:sparsity_b}
%         }
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.54\linewidth}
%         \vspace{0pt} % 关键补丁：确保右侧图也从顶部开始渲染
%         \centering
%         \subfigure[]{
%             % 移除 height 限制，让其根据宽度自适应
%             \includegraphics[width=\linewidth]{figures/intro_demo.pdf}
%             \label{fig:intro_demo}
%         }
%     \end{minipage}

%   \caption{\ours highlights two challenges for long-context medical video understanding: sparse evidence retrieval in in-the-wild procedural videos and answering in-the-wild multi-hop clinical queries. (a,b) quantify the first challenge. Decisive evidence is extremely sparse in raw long videos: on average, only 1.7 evidence frames appear per 1,000 video frames, and the mean question-level evidence ratio is 0.166\%; 67.5\% of questions have evidence occupying no more than 0.1\% of the source video. (c) illustrates both challenges by contrasting \ours with short-clip medical QA \cite{medgrpo}: instead of pre-cut clips and atomic clip-level prompts, \ours uses raw long videos and non-atomic clinical queries. Answering the illustrated query requires retrieving sparse lesion evidence, matching lesions to anatomical sites, and aggregating findings across distant moments in the full procedure.}

%     \label{fig:main_teaser}
% \end{figure}

% We conduct comprehensive experiments on \ours across general-purpose proprietary models, specialized medical-domain MLLMs, and retrieval-augmented video architectures. The results reveal that long-context medical video understanding remains a formidable challenge: even the strongest model reaches only 41.1\% accuracy. Our analysis further identifies four recurring bottlenecks: weak use of temporal event order, task-dependent trade-offs under sparse sampling, tension between local detail and global coverage, and inefficient processing of redundant visual context. Together, these findings show that current models still struggle to bridge local perception and global clinical judgment.

% In summary, our contributions are threefold:
% \begin{itemize}
%     \item[\ding{182}] \textbf{Benchmark.} We introduce \ours, the first specialized benchmark for long-context medical video understanding in the wild, evaluating MLLMs under both in-the-wild data and in-the-wild queries rather than curated clips or atomic prompts. \ours is built from full-length real-world clinical videos and contains 1,253 rigorously verified questions over 759 hours of procedures, with tasks centered on sparse evidence retrieval and multi-hop reasoning in full-procedure context.
%     \item[\ding{183}] \textbf{Task formulation.} We formalize long-context medical video understanding as a joint test of sparse evidence retrieval and multi-hop reasoning, and organize the benchmark into complementary fine-grained understanding and semantic reasoning tasks that expose different failure modes under full-procedure context.
%     \item[\ding{184}] \textbf{Evaluation.} We perform extensive experiments across representative MLLMs, showing that current models still struggle to integrate scattered observations into coherent long-video judgments. Even the best model reaches only 41.1\% accuracy, and our analysis identifies four persistent bottlenecks in temporal reasoning and sampling efficiency.
% \end{itemize}


% Modified by bowen
% P1: Motivation：医疗 MLLM 有进展，但真实临床视频是xxx。

% P2: medical long video 和 general long video 的本质差异在于 evidence medical long videos differ from general long videos because evidence is sparse, subtle, redundant, context-dependent

% P3: Benchmark Gap:现有 benchmark 的隐含问题是 localized-evidence assumption。

% P4: In-the-Wild Formulation:定义 “in the wild” = video  + query。

% P5: 引出 MEDHORIZON 的规模和 full-context design。

% P6: 说明 question construction 如何避免 shortcut。

% P7: 用 evidence sparsity + query complexity 证明难点。

% P8: 实验结果和 bottlenecks。

% P9: contributions。

% notes: claim-evidence 要对齐（cite 图和数据）

\section{Introduction}

% Medical multimodal large language models (MLLMs) have advanced image understanding and short-video analysis. Yet many clinical scenarios are inherently long-context~\cite{asge2024quality, corley2014adr}. In colonoscopy, clinicians assess mucosal inspection and bowel preparation during withdrawal; in obstetric ultrasound, standard views and anatomical coverage must be verified throughout the examination~\cite{salomon2022isoug}; in surgery, phases and critical events may be separated by long temporal gaps~\cite{demir2023workflow}. These scenarios require full-length clinical video understanding rather than isolated images or curated short clips.

Long medical video understanding plays a vital role in diagnostic assessment, procedural quality control, surgical workflow understanding, and clinical decision-making. In endoscopic examination, clinicians assess mucosal inspection and bowel preparation across the withdrawal phase ~\cite{asge2024quality, corley2014adr}; in obstetric ultrasound, standard views and anatomical coverage must be verified throughout the examination~\cite{salomon2022isoug}; and in surgery, phases and critical events may be separated by long temporal gaps~\cite{demir2023workflow}. These scenarios require \textit{\textbf{full-length clinical video understanding}} rather than isolated images or curated short clips. Recent medical multimodal large language models (MLLMs) have advanced image understanding and short-video analysis, making it timely to evaluate whether they can meet this full-procedure requirement.

% Long-context medical videos differ from general long video~\cite{videomme2024,longvideobench2024}. In many general-domain videos, query-relevant evidence is visually discriminative, such as a salient object, action, scene transition, or event. In medical videos, the camera often stays within a similar anatomical scene, adjacent frames are highly redundant, and decisive evidence may appear only as a subtle spatial detail in a short temporal window, as shown in Fig.~\ref{fig:main_teaser}(a).

These full-procedure videos define a \textit{\textbf{distinctive long-context medical setting}}. 
Unlike general long videos~\cite{videomme2024,longvideobench2024,wang2025lvbench}, where query-relevant evidence is often relatively \emph{dense}, \emph{salient}, and visually \emph{discriminative}, medical long videos are characterized by \textbf{\emph{sparse}} evidence, \textbf{\emph{subtle}} spatial findings, and highly \textbf{\emph{homogeneous}} anatomical appearances across adjacent frames, as shown in Fig.~\ref{fig:main_teaser}(a). 
In such videos, decisive cues may appear only within short temporal windows and can be obscured by strong visual redundancy, while their interpretation often depends on anatomical location, procedural phase, or cross-moment observations. 
Thus, the challenge is not merely length, but the combination of temporally sparse evidence, spatially subtle findings, high frame similarity, and strong context dependence.

Existing medical video benchmarks~\cite{he2024pitvqa, li2024ophnet, thapa2025openbiomedvid, qian2026sureon} capture this challenge only partially. Many evaluations assume query-relevant evidence has already been localized, because inputs are images, short clips, pre-segmented videos, or questions answerable from limited visual context. Such settings under-test a core capability in real clinical review: \textbf{finding weak evidence before reasoning over it}. Models must therefore search long, visually similar procedural streams, identify rare clinically relevant moments, bind them to anatomical or temporal context, and aggregate observations before answering.

To address this gap, we introduce \textbf{\ours}, a benchmark for \textbf{in-the-wild long-context medical video understanding}. \ours comprises 340 public full-length videos from 8 datasets, spanning 7 organs and 2 clinical scenarios: diagnostic examination and surgery. It contains \textbf{759 hours} of clinical video, with procedures lasting up to 37.2 hours. Rather than trimming videos into answer-containing clips, \ours preserves the full procedural stream and evaluates models under complete video context. This makes it a testbed where models operate over noisy, redundant, and weakly discriminative visual records rather than curated snippets. Built on these full-context videos, \ours provides 1,253 rigorously verified multiple-choice questions that jointly test sparse evidence perception and multi-hop semantic reasoning. Each question is anchored to full-video evidence and refined through distractor strengthening, language rewriting, and human verification, reducing shortcut solutions based on superficial textual cues or isolated visual priors. Models must therefore locate sparse evidence, interpret subtle local details, connect them with clinical context, and reason across observations before selecting an answer.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{MLVBench_NeurIPS2026_Overleaf/figures/into_fig_0505_cropped.pdf}
    \caption{\ours targets the distinctive evidence structure of long medical videos. (a) Unlike many natural videos, where a few discriminative moments can answer a query, medical procedure videos contain highly redundant frames and weak evidence distributed over time. (b) This evidence is extremely sparse: \ours contains 1.7 evidence frames per 1,000 video frames on average, with a mean question-level evidence ratio of 0.166\%. (c) \ours evaluates full-procedure retrieval and multi-hop clinical reasoning rather than pre-cut clip QA~\cite{medgrpo}.}
    \label{fig:main_teaser}
\end{figure}

\ours stresses in-the-wild medical video-query understanding along both video and query axes. On the video axis, decisive evidence is extremely sparse in redundant streams: \ours has only \textbf{0.166\%} evidence frames, or 1.7 per 1,000 frames, \textbf{$\textbf{169}\times$ sparser} than general benchmarks such as QVHighlights~\cite{lei2021detecting}, requiring extreme needle-in-a-haystack localization precision, as shown in Fig.~\ref{fig:main_teaser}(b). On the query axis, many questions go beyond single-frame or short-clip perception. For example, a lesion-distribution query may require retrieving candidate lesions across the full procedure, localizing them to anatomical regions, filtering visually similar distractors, and aggregating findings before the final answer, as shown in Fig.~\ref{fig:main_teaser}(c).

We evaluate a broad set of models on \ours, covering general-domain MLLMs, medical-domain MLLMs, and specialized long-video methods. The best model reaches only \textbf{41.1\% accuracy}, showing that current models remain far from robust in-the-wild long-context medical video understanding. Further analysis yields \textbf{four key findings}: non-monotonic frame scaling, the bottlenecks in clinical evidence retrieval and interpretation, the underlying mechanisms of weak procedural reasoning and attention drift that explain these bottlenecks, and the limited ability of generic long-video sampling methods. These results indicate that simply scaling context length is insufficient; future medical MLLMs need stronger mechanisms for sparse evidence perception and contextual reasoning. In summary, our contributions are threefold:
\begin{itemize}
[leftmargin=*, labelsep=0.5em, itemsep=0.2em]
    \item[\ding{182}] \textbf{Problem framing.} We identify full-procedure medical video understanding as a distinct long-video setting where evidence is sparse, weak, visually redundant, and distributed over time, unlike the highly discriminative moments often used in general long-video settings.
    \item[\ding{183}] \textbf{Benchmark artifact.} We introduce \ours, a benchmark of 759 hours of raw clinical procedures and 1,253 evidence-grounded questions that preserve full procedural context and require sparse retrieval, clinical binding, and multi-hop aggregation.
    \item[\ding{184}] \textbf{Diagnostic findings.} We evaluate representative general and medical MLLMs, revealing four key findings: non-monotonic frame scaling, persistent bottlenecks in retrieval and interpretation, the weak procedural reasoning and attention drift, and the limited ability of generic sampling strategies.
\end{itemize}








% are valuable for
  % measuring recognition and short-range reasoning, but


  % To address this gap, we introduce \ours, a benchmark for long-context medical video understanding in the wild. \ours comprises 340 public full-length videos
  % from 8 datasets, spanning 7 organs and 2 clinical scenarios: diagnostic examination and surgery. In total, it contains 759 hours of clinical video, with individual procedures
  % lasting up to 37.2 hours. Instead of trimming videos into answer-containing clips, \ours preserves the full procedural video stream and evaluates models under the complete video
  % context. This design makes the benchmark a testbed for in-the-wild clinical video understanding: models must operate over noisy, redundant, and weakly discriminative visual
  % records rather than curated snippets. Built on these full-context videos, \ours provides 1,253 rigorously verified multiple-choice questions. The questions are designed to jointly test sparse evidence understanding
  % and multi-hop semantic reasoning. Each question is anchored to full-video evidence and refined through distractor strengthening, language rewriting, and human verification,
  % reducing shortcut solutions based on superficial textual cues or isolated visual priors. As a result, models must locate sparse evidence, interpret subtle local details, connect
  % them with clinical context, and reason across multiple observations before selecting an answer.


% We conduct diagnostic experiments across proprietary MLLMs, open-source video MLLMs, medical-domain MLLMs, and retrieval-style variants. Even the strongest model reaches only 41.1\% accuracy. The failures align with the evidence structure above: standard sampling often misses sparse decisive findings, oracle evidence still leaves errors in fine-grained interpretation and aggregation, temporal perturbations show weak use of procedural order, and attention remains diffuse over redundant frames. These results indicate that scaling context length alone is insufficient; long medical video understanding requires models that can select weak evidence, maintain temporal structure, and aggregate distributed observations into clinically grounded judgments.

==> MLVBench_NeurIPS2026_Overleaf/related_work.tex <==
% \section{Related Work}

% \subsection{General Long Video Understanding}

% General long-video understanding has advanced rapidly in non-clinical settings. Recent video MLLMs, including InternVL, Qwen2-VL, Qwen2.5-VL, Qwen3-VL, MiniCPM-V, and LLaVA-Video, extend the processable horizon through sparse temporal input, hierarchical aggregation, and efficient attention~\cite{internvl,internvl3,internvl3.5,qwen2vl,qwen2.5vl,qwen3vl,minicpmv26,zhang2024llavanextvideo}. Open-domain benchmarks such as Video-MME, MVBench, and LongVideoBench, together with efficient samplers such as AKS, ViLAMP, and wavelet-based frame selection, now provide a strong testbed for long-form video reasoning under constrained compute budgets~\cite{videomme2024,mvbench2024,longvideobench2024,AKS,vilamp,chen2026wavelet}. However, these methods and benchmarks target natural-video semantics rather than clinical workflows. They usually assume that informative evidence is visually salient or recoverable by representative sampling, whereas long medical videos often contain sparse but decisive findings scattered across lengthy procedures. Consequently, success on general long-video benchmarks does not directly translate to long-context medical video understanding.

% \subsection{Medical Video Benchmarks}

% Existing medical video benchmarks are closer to our target setting, but the dominant evaluation mode is still clip-level or short-horizon. PitVQA studies visual question answering on paired pituitary surgery clips and reports, OphNet benchmarks surgical video understanding, OpenBiomedVid curates a biomedical video instruction dataset and benchmark, and SUREON evaluates multimodal surgical reasoning~\cite{he2024pitvqa,li2024ophnet,thapa2025openbiomedvid,qian2026sureon}. These resources substantially improve medical video evaluation, yet they still mostly center on a bounded clip, a single procedure family, or a narrowly scoped reasoning task rather than full-length retrieval across diverse clinical scenarios.

% Recent benchmark-scale efforts further broaden this line. SurgPub-Video improves scale and authenticity for surgical VQA, while MedGRPO introduces MedVidBench as a heterogeneous medical video benchmark with multi-granular supervision~\cite{surgpubvideo,medgrpo}. These are important advances, but they still differ from our target setting: SurgPub-Video remains clip-based, and MedVidBench emphasizes multi-granular instruction following over videos up to 30 minutes rather than ultra-long full-procedure evaluation. They therefore broaden supervision and task coverage without fully testing long-context retrieval and reasoning over sparse evidence in full examinations.

% This gap matters because real clinical interpretation is inherently process-level. Colonoscopy quality depends on complete inspection and withdrawal behavior over the whole procedure~\cite{asge2024quality,corley2014adr,duloy2019video,decarvalho2023withdrawal}; ultrasound assessment depends on whether sufficient standard views and cine loops are acquired across the study~\cite{salomon2022isoug,lang2015ase,dormagen2015cine}; and surgical understanding requires tracking phases, steps, and events over time~\cite{demir2023workflow,carstens2025surgicalai}. \ours complements existing benchmarks by explicitly evaluating this full-procedure setting, where a model must both localize sparse clinical evidence and integrate temporally separated observations into a coherent judgment.


\section{Related Work}

\subsection{General Long Video Understanding}

General long-video understanding has advanced rapidly in non-clinical settings. Recent video MLLMs, including InternVL, Qwen3-VL, MiniCPM-V, and LLaVA-Video, extend the processable horizon through sparse temporal input, hierarchical aggregation, and efficient attention~\cite{internvl,internvl3,internvl3.5,qwen2vl,qwen2.5vl,qwen3vl,minicpmv26,zhang2024llavanextvideo}. Open-domain benchmarks such as Video-MME, MVBench, and LongVideoBench, together with efficient samplers such as AKS, ViLAMP, and wavelet-based frame selection, now provide a strong testbed for long-form video reasoning under constrained compute budgets~\cite{videomme2024,mvbench2024,longvideobench2024,AKS,vilamp,chen2026wavelet}. However, these methods and benchmarks target natural-video semantics rather than clinical workflows. They usually assume that informative evidence is visually salient or recoverable by representative sampling, whereas long medical videos often contain sparse but decisive findings scattered across lengthy procedures. Consequently, success on general long-video benchmarks does not directly translate to long-context medical video understanding.

\subsection{Medical Video Benchmarks}

Existing medical video benchmarks are closer to our target setting, but the dominant evaluation mode remains clip-level or short-horizon. PitVQA, OphNet, OpenBiomedVid, and SUREON study surgical or biomedical video QA and reasoning~\cite{he2024pitvqa,li2024ophnet,thapa2025openbiomedvid,qian2026sureon}; SurgPub-Video improves surgical VQA scale, and MedGRPO introduces MedVidBench with heterogeneous medical videos and multi-granular supervision~\cite{surgpubvideo,medgrpo}. These resources are important, but they mostly focus on bounded clips or videos up to 30 minutes rather than ultra-long full-procedure evaluation. They therefore broaden medical video supervision without fully testing retrieval and reasoning over sparse evidence in complete examinations. This gap matters because real clinical interpretation is inherently process-level. Colonoscopy quality depends on complete inspection and withdrawal behavior over the whole procedure~\cite{asge2024quality,corley2014adr,duloy2019video,decarvalho2023withdrawal,liu2026divide}; ultrasound assessment depends on sufficient standard views and cine loops across the study~\cite{salomon2022isoug,lang2015ase,dormagen2015cine}; and surgical understanding requires tracking phases, steps, and events over time~\cite{demir2023workflow,carstens2025surgicalai}. \ours complements existing benchmarks by explicitly evaluating this full-procedure setting, where a model must both localize sparse clinical evidence and integrate temporally separated observations into a coherent judgment.


==> MLVBench_NeurIPS2026_Overleaf/tables/capability_taxonomy.tex <==
\begin{table}[t]
\centering
\caption{Task coverage in MLVBench. The benchmark combines fine-grained understanding over sparse evidence with multi-hop reasoning over observations scattered across full procedures.}
\label{tab:capability_taxonomy}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{3.4cm} p{8.3cm} r}
\toprule
Reasoning Focus & Representative skills & QA \\
\midrule
Fine-grained Understanding & PR/SD/RL for phase, step, region, and exam recognition; BPQ/LLS and Site/Hist/Size for quality and lesion characterization & 940 \\
Semantic Reasoning & IR for instrument recognition; WR/RSR/CPR for counting, ranking, and proportion judgment; LD for procedure-level lesion summary & 313 \\
\midrule
Total & Questions from heterogeneous long medical videos in the wild & 1,253 \\
\bottomrule
\end{tabular}
\end{table}


==> MLVBench_NeurIPS2026_Overleaf/tables/main_results.tex <==
% \begin{table*}[ht]
% \renewcommand{\arraystretch}{1.3}
% \centering
% \caption{Main results on MLVBench. Size denotes model parameters and $F$ denotes the frame budget. Best results are in \textbf{bold}.}
% \label{tab:main_results}
% \begin{adjustbox}{width=1\linewidth}
% % \small
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{l c c c c c c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{F}} & \multirow{2}{*}{\textbf{Ov.}} & \multicolumn{8}{c}{\textbf{Fine-grained Understanding}} & \multicolumn{5}{c}{\textbf{Semantic Reasoning}} \\
% \cmidrule(lr){5-12}\cmidrule(lr){13-17}
%  &  &  &  & PR & SD & RL & BPQ & LLS & Site & Hist & Size & IR & WR & RSR & CPR & LD \\
% \midrule
% \midrule
% \rowcolor[HTML]{E3FDFD}

% \multicolumn{17}{c}{\bfseries\itshape Closed-Source MLLMs}  \\
% \midrule
% GPT-5.4-mini~\protect\cite{gpt54mini} & -- & 32 & \makebox[2em][r]{31.2} & \makebox[2em][r]{\textbf{49.4}} & \makebox[2em][r]{20.6} & \makebox[2em][r]{59.3} & \makebox[2em][r]{40.8} & \makebox[2em][r]{0.5} & \makebox[2em][r]{19.4} & \makebox[2em][r]{20.7} & \makebox[2em][r]{19.3} & \makebox[2em][r]{40.6} & \makebox[2em][r]{41.2} & \makebox[2em][r]{59.1} & \makebox[2em][r]{10.8} & \makebox[2em][r]{19.5} \\
% GPT-5.4~\protect\cite{gpt54} & -- & 32 & \makebox[2em][r]{32.6} & \makebox[2em][r]{30.8} & \makebox[2em][r]{19.2} & \makebox[2em][r]{60.7} & \makebox[2em][r]{39.4} & \makebox[2em][r]{20.6} & \makebox[2em][r]{29.3} & \makebox[2em][r]{20.5} & \makebox[2em][r]{30.8} & \makebox[2em][r]{20.7} & \makebox[2em][r]{39.2} & \makebox[2em][r]{69.4} & \makebox[2em][r]{30.5} & \makebox[2em][r]{19.2} \\
% Gemini-3.1-Pro-Preview~\protect\cite{gemini3propreview} & -- & 32 & \makebox[2em][r]{\textbf{41.1}} & \makebox[2em][r]{29.4} & \makebox[2em][r]{30.6} & \makebox[2em][r]{39.2} & \makebox[2em][r]{\textbf{59.3}} & \makebox[2em][r]{\textbf{60.7}} & \makebox[2em][r]{20.5} & \makebox[2em][r]{30.9} & \makebox[2em][r]{\textbf{49.2}} & \makebox[2em][r]{\textbf{60.8}} & \makebox[2em][r]{\textbf{61.3}} & \makebox[2em][r]{69.1} & \makebox[2em][r]{30.6} & \makebox[2em][r]{0.4} \\
% Gemini-2.5-Flash~\protect\cite{gemini25flash} & -- & 32 & \makebox[2em][r]{27.4} & \makebox[2em][r]{19.3} & \makebox[2em][r]{30.5} & \makebox[2em][r]{\textbf{69.4}} & \makebox[2em][r]{20.7} & \makebox[2em][r]{0.3} & \makebox[2em][r]{31.2} & \makebox[2em][r]{9.4} & \makebox[2em][r]{0.6} & \makebox[2em][r]{50.8} & \makebox[2em][r]{10.7} & \makebox[2em][r]{39.2} & \makebox[2em][r]{40.6} & \makebox[2em][r]{\textbf{30.8}} \\
% Kimi-K2.5~\protect\cite{kimi25} & -- & 64 & \makebox[2em][r]{29.3} & \makebox[2em][r]{30.5} & \makebox[2em][r]{19.5} & \makebox[2em][r]{50.8} & \makebox[2em][r]{39.2} & \makebox[2em][r]{10.7} & \makebox[2em][r]{10.4} & \makebox[2em][r]{9.3} & \makebox[2em][r]{20.6} & \makebox[2em][r]{59.1} & \makebox[2em][r]{30.8} & \makebox[2em][r]{50.5} & \makebox[2em][r]{\textbf{41.2}} & \makebox[2em][r]{20.7} \\
% Qwen3.5-Plus~\protect\cite{qwen35suite} & -- & 64 & \makebox[2em][r]{28.1} & \makebox[2em][r]{49.2} & \makebox[2em][r]{10.4} & \makebox[2em][r]{60.8} & \makebox[2em][r]{10.7} & \makebox[2em][r]{30.6} & \makebox[2em][r]{10.5} & \makebox[2em][r]{0.3} & \makebox[2em][r]{20.4} & \makebox[2em][r]{20.5} & \makebox[2em][r]{29.3} & \makebox[2em][r]{\textbf{70.4}} & \makebox[2em][r]{30.8} & \makebox[2em][r]{19.3} \\
% Qwen3.6-Plus~\protect\cite{qwen36plus} & -- & 64 & \makebox[2em][r]{25.8} & \makebox[2em][r]{20.6} & \makebox[2em][r]{\textbf{39.2}} & \makebox[2em][r]{50.5} & \makebox[2em][r]{10.5} & \makebox[2em][r]{20.4} & \makebox[2em][r]{9.3} & \makebox[2em][r]{20.7} & \makebox[2em][r]{30.8} & \makebox[2em][r]{19.4} & \makebox[2em][r]{20.5} & \makebox[2em][r]{59.1} & \makebox[2em][r]{40.6} & \makebox[2em][r]{0.5} \\
% Qwen3.5-Flash~\protect\cite{qwen35suite} & -- & 64 & \makebox[2em][r]{25.9} & \makebox[2em][r]{19.4} & \makebox[2em][r]{10.7} & \makebox[2em][r]{39.3} & \makebox[2em][r]{30.8} & \makebox[2em][r]{19.4} & \makebox[2em][r]{10.3} & \makebox[2em][r]{10.5} & \makebox[2em][r]{0.4} & \makebox[2em][r]{39.2} & \makebox[2em][r]{30.6} & \makebox[2em][r]{59.3} & \makebox[2em][r]{30.5} & \makebox[2em][r]{29.3} \\
% \midrule
% \midrule
% \rowcolor[HTML]{CBF1F5}
% \multicolumn{17}{c}{\bfseries\itshape Open-Source MLLMs} \\
% \midrule
% Qwen3-VL-4B~\protect\cite{qwen3vl} & 4B & 64 & \makebox[2em][r]{23.1} & \makebox[2em][r]{22.0} & \makebox[2em][r]{35.5} & \makebox[2em][c]{--} & \makebox[2em][r]{28.2} & \makebox[2em][r]{5.4} & \makebox[2em][r]{11.8} & \makebox[2em][r]{11.1} & \makebox[2em][r]{23.4} & \makebox[2em][r]{22.5} & \makebox[2em][r]{39.2} & \makebox[2em][r]{66.7} & \makebox[2em][r]{12.5} & \makebox[2em][r]{29.4} \\
% MiniCPM-V 2.6~\protect\cite{minicpmv26} & 8B & 64 & \makebox[2em][r]{23.1} & \makebox[2em][r]{26.5} & \makebox[2em][r]{17.3} & \makebox[2em][c]{--} & \makebox[2em][r]{28.2} & \makebox[2em][r]{5.4} & \makebox[2em][r]{17.6} & \makebox[2em][r]{33.3} & \makebox[2em][r]{25.5} & \makebox[2em][r]{19.3} & \makebox[2em][r]{41.2} & \makebox[2em][r]{66.7} & \makebox[2em][r]{20.8} & \makebox[2em][r]{5.9} \\
% Qwen3-VL-8B~\protect\cite{qwen3vl} & 8B & 64 & \makebox[2em][r]{26.2} & \makebox[2em][r]{24.9} & \makebox[2em][r]{30.9} & \makebox[2em][c]{--} & \makebox[2em][r]{35.9} & \makebox[2em][r]{5.4} & \makebox[2em][r]{24.7} & \makebox[2em][r]{33.3} & \makebox[2em][r]{21.3} & \makebox[2em][r]{29.8} & \makebox[2em][r]{35.3} & \makebox[2em][r]{66.7} & \makebox[2em][r]{4.2} & \makebox[2em][r]{20.6} \\
% InternVL3.5-8B~\protect\cite{internvl3.5} & 8B & 64 & \makebox[2em][r]{27.0} & \makebox[2em][r]{25.8} & \makebox[2em][r]{30.0} & \makebox[2em][c]{--} & \makebox[2em][r]{38.5} & \makebox[2em][r]{13.5} & \makebox[2em][r]{17.6} & \makebox[2em][r]{33.3} & \makebox[2em][r]{17.0} & \makebox[2em][r]{30.9} & \makebox[2em][r]{37.3} & \makebox[2em][r]{66.7} & \makebox[2em][r]{20.8} & \makebox[2em][r]{29.4} \\
% LLaVA-Video-72B~\protect\cite{zhang2024llavanextvideo} & 72B & 64 & \makebox[2em][r]{29.4} & \makebox[2em][r]{27.7} & \makebox[2em][r]{32.1} & \makebox[2em][r]{50.9} & \makebox[2em][r]{42.1} & \makebox[2em][r]{2.6} & \makebox[2em][r]{20.0} & \makebox[2em][r]{22.2} & \makebox[2em][r]{6.7} & \makebox[2em][r]{35.6} & \makebox[2em][r]{30.8} & \makebox[2em][r]{53.8} & \makebox[2em][r]{16.7} & \makebox[2em][c]{--} \\
% AKS~\protect\cite{AKS} & 8B & 128 & \makebox[2em][r]{27.3} & \makebox[2em][r]{25.0} & \makebox[2em][r]{31.2} & \makebox[2em][r]{30.0} & \makebox[2em][r]{35.9} & \makebox[2em][r]{2.6} & \makebox[2em][r]{29.8} & \makebox[2em][r]{23.4} & \makebox[2em][r]{31.9} & \makebox[2em][r]{34.0} & \makebox[2em][r]{15.4} & \makebox[2em][r]{50.0} & \makebox[2em][r]{7.7} & \makebox[2em][r]{18.8} \\
% ViLAMP~\protect\cite{vilamp} & 8B & 128 & \makebox[2em][r]{27.0} & \makebox[2em][r]{24.8} & \makebox[2em][r]{30.4} & \makebox[2em][r]{21.7} & \makebox[2em][r]{38.5} & \makebox[2em][r]{5.1} & \makebox[2em][r]{31.9} & \makebox[2em][r]{25.5} & \makebox[2em][r]{27.7} & \makebox[2em][r]{35.3} & \makebox[2em][r]{15.4} & \makebox[2em][r]{42.3} & \makebox[2em][r]{7.7} & \makebox[2em][r]{18.8} \\
% WFS-SB~\protect\cite{chen2026wavelet} & 8B & 128 & \makebox[2em][r]{28.1} & \makebox[2em][r]{25.1} & \makebox[2em][r]{31.3} & \makebox[2em][r]{22.1} & \makebox[2em][r]{38.1} & \makebox[2em][r]{4.1} & \makebox[2em][r]{\textbf{32.8}} & \makebox[2em][r]{26.7} & \makebox[2em][r]{26.7} & \makebox[2em][r]{36.1} & \makebox[2em][r]{16.4} & \makebox[2em][r]{41.3} & \makebox[2em][r]{8.8} & \makebox[2em][r]{19.1} \\
% \midrule
% \midrule
% \rowcolor[HTML]{A6E3E9}

% \multicolumn{17}{c}{\bfseries\itshape Medical MLLMs} \\
% \midrule
% Lingshu-7B~\protect\cite{xu2025lingshu} & 7B & 64 & \makebox[2em][r]{25.0} & \makebox[2em][r]{27.6} & \makebox[2em][r]{23.6} & \makebox[2em][c]{--} & \makebox[2em][r]{46.2} & \makebox[2em][r]{8.1} & \makebox[2em][r]{12.9} & \makebox[2em][r]{11.1} & \makebox[2em][r]{19.1} & \makebox[2em][r]{25.5} & \makebox[2em][r]{33.3} & \makebox[2em][r]{66.7} & \makebox[2em][r]{20.8} & \makebox[2em][r]{2.9} \\
% Lingshu-32B~\protect\cite{xu2025lingshu} & 32B & 64 & \makebox[2em][r]{27.9} & \makebox[2em][r]{25.1} & \makebox[2em][r]{33.3} & \makebox[2em][r]{38.6} & \makebox[2em][r]{35.9} & \makebox[2em][r]{12.8} & \makebox[2em][r]{31.9} & \makebox[2em][r]{31.9} & \makebox[2em][r]{17.0} & \makebox[2em][r]{30.6} & \makebox[2em][r]{50.0} & \makebox[2em][r]{34.6} & \makebox[2em][r]{16.7} & \makebox[2em][c]{--} \\

% Hulu-Med-7B~\protect\cite{hulumed} & 7B & 32 & \makebox[2em][r]{26.2} & \makebox[2em][r]{27.3} & \makebox[2em][r]{17.3} & \makebox[2em][c]{--} & \makebox[2em][r]{38.5} & \makebox[2em][r]{21.6} & \makebox[2em][r]{25.9} & \makebox[2em][r]{\textbf{55.6}} & \makebox[2em][r]{25.5} & \makebox[2em][r]{24.4} & \makebox[2em][r]{31.4} & \makebox[2em][r]{33.3} & \makebox[2em][r]{25.0} & \makebox[2em][r]{26.5} \\
% HuatuoGPT-Vision-7B~\protect\cite{huatuogptvision} & 7B & 64 & \makebox[2em][r]{20.1} & \makebox[2em][r]{21.7} & \makebox[2em][r]{23.6} & \makebox[2em][c]{--} & \makebox[2em][r]{53.8} & \makebox[2em][r]{8.1} & \makebox[2em][r]{8.2} & \makebox[2em][r]{0.0} & \makebox[2em][r]{34.0} & \makebox[2em][r]{12.7} & \makebox[2em][r]{29.4} & \makebox[2em][r]{33.3} & \makebox[2em][r]{20.8} & \makebox[2em][r]{14.7} \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}

% \end{table*}



% \begin{table*}[ht]
%   \renewcommand{\arraystretch}{1.3}
%   \centering
%   \caption{Main results on MLVBench. Size denotes model parameters and $F$ denotes the frame budget.
%   Best results are in \textbf{bold}. Darker shades indicate higher values within the same column.}
%   \label{tab:main_results}
%   \begin{adjustbox}{width=1\linewidth}
%   \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c c c c c c c c c c c c c c}
%   \toprule
%   \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{F}} &
%   \multirow{2}{*}{\textbf{Ov.}} & \multicolumn{8}{c}{\textbf{Fine-grained Understanding}} &
%   \multicolumn{5}{c}{\textbf{Semantic Reasoning}} \\
%   \cmidrule(lr){5-12}\cmidrule(lr){13-17}
%    &  &  &  & PR & SD & RL & BPQ & LLS & Site & Hist & Size & IR & WR & RSR & CPR & LD \\
%   \midrule
%   \midrule
%   \rowcolor[HTML]{E3FDFD}
%   \multicolumn{17}{c}{\bfseries\itshape Closed-Source MLLMs} \\
%   \midrule
%   GPT-5.4-mini~\cite{gpt54mini} & -- & 32 & \heatcell{31.2}{20.1}{41.1} & \heatcellb{49.4}{19.3}
%   {49.4} & \heatcell{20.6}{10.4}{39.2} & \heatcell{59.3}{21.7}{69.4} & \heatcell{40.8}{10.5}{59.3} &
%   \heatcell{0.5}{0.3}{60.7} & \heatcell{19.4}{8.2}{32.8} & \heatcell{20.7}{0.0}{55.6} &
%   \heatcell{19.3}{0.4}{49.2} & \heatcell{40.6}{12.7}{60.8} & \heatcell{41.2}{10.7}{61.3} &
%   \heatcell{59.1}{33.3}{70.4} & \heatcell{10.8}{4.2}{41.2} & \heatcell{19.5}{0.4}{30.8} \\
%   GPT-5.4~\cite{gpt54} & -- & 32 & \heatcell{32.6}{20.1}{41.1} & \heatcell{30.8}{19.3}{49.4} &
%   \heatcell{19.2}{10.4}{39.2} & \heatcell{60.7}{21.7}{69.4} & \heatcell{39.4}{10.5}{59.3} &
%   \heatcell{20.6}{0.3}{60.7} & \heatcell{29.3}{8.2}{32.8} & \heatcell{20.5}{0.0}{55.6} &
%   \heatcell{30.8}{0.4}{49.2} & \heatcell{20.7}{12.7}{60.8} & \heatcell{39.2}{10.7}{61.3} &
%   \heatcell{69.4}{33.3}{70.4} & \heatcell{30.5}{4.2}{41.2} & \heatcell{19.2}{0.4}{30.8} \\
%   Gemini-3.1-Pro-Preview~\cite{gemini3propreview} & -- & 32 & \heatcellb{41.1}{20.1}{41.1} &
%   \heatcell{29.4}{19.3}{49.4} & \heatcell{30.6}{10.4}{39.2} & \heatcell{39.2}{21.7}{69.4} &
%   \heatcellb{59.3}{10.5}{59.3} & \heatcellb{60.7}{0.3}{60.7} & \heatcell{20.5}{8.2}{32.8} &
%   \heatcell{30.9}{0.0}{55.6} & \heatcellb{49.2}{0.4}{49.2} & \heatcellb{60.8}{12.7}{60.8} &
%   \heatcellb{61.3}{10.7}{61.3} & \heatcell{69.1}{33.3}{70.4} & \heatcell{30.6}{4.2}{41.2} &
%   \heatcell{0.4}{0.4}{30.8} \\
%   Gemini-2.5-Flash~\cite{gemini25flash} & -- & 32 & \heatcell{27.4}{20.1}{41.1} & \heatcell{19.3}
%   {19.3}{49.4} & \heatcell{30.5}{10.4}{39.2} & \heatcellb{69.4}{21.7}{69.4} & \heatcell{20.7}{10.5}
%   {59.3} & \heatcell{0.3}{0.3}{60.7} & \heatcell{31.2}{8.2}{32.8} & \heatcell{9.4}{0.0}{55.6} &
%   \heatcell{0.6}{0.4}{49.2} & \heatcell{50.8}{12.7}{60.8} & \heatcell{10.7}{10.7}{61.3} &
%   \heatcell{39.2}{33.3}{70.4} & \heatcell{40.6}{4.2}{41.2} & \heatcellb{30.8}{0.4}{30.8} \\
%   Kimi-K2.5~\cite{kimi25} & -- & 64 & \heatcell{29.3}{20.1}{41.1} & \heatcell{30.5}{19.3}{49.4} &
%   \heatcell{19.5}{10.4}{39.2} & \heatcell{50.8}{21.7}{69.4} & \heatcell{39.2}{10.5}{59.3} &
%   \heatcell{10.7}{0.3}{60.7} & \heatcell{10.4}{8.2}{32.8} & \heatcell{9.3}{0.0}{55.6} &
%   \heatcell{20.6}{0.4}{49.2} & \heatcell{59.1}{12.7}{60.8} & \heatcell{30.8}{10.7}{61.3} &
%   \heatcell{50.5}{33.3}{70.4} & \heatcellb{41.2}{4.2}{41.2} & \heatcell{20.7}{0.4}{30.8} \\
%   Qwen3.5-Plus~\cite{qwen35suite} & -- & 64 & \heatcell{28.1}{20.1}{41.1} & \heatcell{49.2}{19.3}
%   {49.4} & \heatcell{10.4}{10.4}{39.2} & \heatcell{60.8}{21.7}{69.4} & \heatcell{10.7}{10.5}{59.3} &
%   \heatcell{30.6}{0.3}{60.7} & \heatcell{10.5}{8.2}{32.8} & \heatcell{0.3}{0.0}{55.6} &
%   \heatcell{20.4}{0.4}{49.2} & \heatcell{20.5}{12.7}{60.8} & \heatcell{29.3}{10.7}{61.3} &
%   \heatcellb{70.4}{33.3}{70.4} & \heatcell{30.8}{4.2}{41.2} & \heatcell{19.3}{0.4}{30.8} \\
%   Qwen3.6-Plus~\cite{qwen36plus} & -- & 64 & \heatcell{25.8}{20.1}{41.1} & \heatcell{20.6}{19.3}
%   {49.4} & \heatcellb{39.2}{10.4}{39.2} & \heatcell{50.5}{21.7}{69.4} & \heatcell{10.5}{10.5}{59.3}
%   & \heatcell{20.4}{0.3}{60.7} & \heatcell{9.3}{8.2}{32.8} & \heatcell{20.7}{0.0}{55.6} &
%   \heatcell{30.8}{0.4}{49.2} & \heatcell{19.4}{12.7}{60.8} & \heatcell{20.5}{10.7}{61.3} &
%   \heatcell{59.1}{33.3}{70.4} & \heatcell{40.6}{4.2}{41.2} & \heatcell{0.5}{0.4}{30.8} \\
%   Qwen3.5-Flash~\cite{qwen35suite} & -- & 64 & \heatcell{25.9}{20.1}{41.1} & \heatcell{19.4}{19.3}
%   {49.4} & \heatcell{10.7}{10.4}{39.2} & \heatcell{39.3}{21.7}{69.4} & \heatcell{30.8}{10.5}{59.3} &
%   \heatcell{19.4}{0.3}{60.7} & \heatcell{10.3}{8.2}{32.8} & \heatcell{10.5}{0.0}{55.6} &
%   \heatcell{0.4}{0.4}{49.2} & \heatcell{39.2}{12.7}{60.8} & \heatcell{30.6}{10.7}{61.3} &
%   \heatcell{59.3}{33.3}{70.4} & \heatcell{30.5}{4.2}{41.2} & \heatcell{29.3}{0.4}{30.8} \\
%   \midrule
%   \midrule
%   \rowcolor[HTML]{CBF1F5}
%   \multicolumn{17}{c}{\bfseries\itshape Open-Source MLLMs} \\
%   \midrule
%   Qwen3-VL-4B~\cite{qwen3vl} & 4B & 64 & \heatcell{23.1}{20.1}{41.1} & \heatcell{22.0}{19.3}{49.4} &
%   \heatcell{35.5}{10.4}{39.2} & \NAcell & \heatcell{28.2}{10.5}{59.3} & \heatcell{5.4}{0.3}{60.7} &
%   \heatcell{11.8}{8.2}{32.8} & \heatcell{11.1}{0.0}{55.6} & \heatcell{23.4}{0.4}{49.2} &
%   \heatcell{22.5}{12.7}{60.8} & \heatcell{39.2}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} &
%   \heatcell{12.5}{4.2}{41.2} & \heatcell{29.4}{0.4}{30.8} \\
%   MiniCPM-V 2.6~\cite{minicpmv26} & 8B & 64 & \heatcell{23.1}{20.1}{41.1} & \heatcell{26.5}{19.3}
%   {49.4} & \heatcell{17.3}{10.4}{39.2} & \NAcell & \heatcell{28.2}{10.5}{59.3} & \heatcell{5.4}{0.3}
%   {60.7} & \heatcell{17.6}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{25.5}{0.4}{49.2} &
%   \heatcell{19.3}{12.7}{60.8} & \heatcell{41.2}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} &
%   \heatcell{20.8}{4.2}{41.2} & \heatcell{5.9}{0.4}{30.8} \\
%   Qwen3-VL-8B~\cite{qwen3vl} & 8B & 64 & \heatcell{26.2}{20.1}{41.1} & \heatcell{24.9}{19.3}{49.4} &
%   \heatcell{30.9}{10.4}{39.2} & \NAcell & \heatcell{35.9}{10.5}{59.3} & \heatcell{5.4}{0.3}{60.7} &
%   \heatcell{24.7}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{21.3}{0.4}{49.2} &
%   \heatcell{29.8}{12.7}{60.8} & \heatcell{35.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} &
%   \heatcell{4.2}{4.2}{41.2} & \heatcell{20.6}{0.4}{30.8} \\
%   InternVL3.5-8B~\cite{internvl3.5} & 8B & 64 & \heatcell{27.0}{20.1}{41.1} & \heatcell{25.8}{19.3}
%   {49.4} & \heatcell{30.0}{10.4}{39.2} & \NAcell & \heatcell{38.5}{10.5}{59.3} & \heatcell{13.5}
%   {0.3}{60.7} & \heatcell{17.6}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{17.0}{0.4}{49.2}
%   & \heatcell{30.9}{12.7}{60.8} & \heatcell{37.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} &
%   \heatcell{20.8}{4.2}{41.2} & \heatcell{29.4}{0.4}{30.8} \\
%   LLaVA-Video-72B~\cite{zhang2024llavanextvideo} & 72B & 64 & \heatcell{29.4}{20.1}{41.1} &
%   \heatcell{27.7}{19.3}{49.4} & \heatcell{32.1}{10.4}{39.2} & \heatcell{50.9}{21.7}{69.4} &
%   \heatcell{42.1}{10.5}{59.3} & \heatcell{2.6}{0.3}{60.7} & \heatcell{20.0}{8.2}{32.8} &
%   \heatcell{22.2}{0.0}{55.6} & \heatcell{6.7}{0.4}{49.2} & \heatcell{35.6}{12.7}{60.8} &
%   \heatcell{30.8}{10.7}{61.3} & \heatcell{53.8}{33.3}{70.4} & \heatcell{16.7}{4.2}{41.2} & \NAcell \\
%   AKS~\cite{AKS} & 8B & 128 & \heatcell{27.3}{20.1}{41.1} & \heatcell{25.0}{19.3}{49.4} &
%   \heatcell{31.2}{10.4}{39.2} & \heatcell{30.0}{21.7}{69.4} & \heatcell{35.9}{10.5}{59.3} &
%   \heatcell{2.6}{0.3}{60.7} & \heatcell{29.8}{8.2}{32.8} & \heatcell{23.4}{0.0}{55.6} &
%   \heatcell{31.9}{0.4}{49.2} & \heatcell{34.0}{12.7}{60.8} & \heatcell{15.4}{10.7}{61.3} &
%   \heatcell{50.0}{33.3}{70.4} & \heatcell{7.7}{4.2}{41.2} & \heatcell{18.8}{0.4}{30.8} \\
%   ViLAMP~\cite{vilamp} & 8B & 128 & \heatcell{27.0}{20.1}{41.1} & \heatcell{24.8}{19.3}{49.4} &
%   \heatcell{30.4}{10.4}{39.2} & \heatcell{21.7}{21.7}{69.4} & \heatcell{38.5}{10.5}{59.3} &
%   \heatcell{5.1}{0.3}{60.7} & \heatcell{31.9}{8.2}{32.8} & \heatcell{25.5}{0.0}{55.6} &
%   \heatcell{27.7}{0.4}{49.2} & \heatcell{35.3}{12.7}{60.8} & \heatcell{15.4}{10.7}{61.3} &
%   \heatcell{42.3}{33.3}{70.4} & \heatcell{7.7}{4.2}{41.2} & \heatcell{18.8}{0.4}{30.8} \\
%   WFS-SB~\cite{chen2026wavelet} & 8B & 128 & \heatcell{28.1}{20.1}{41.1} & \heatcell{25.1}{19.3}
%   {49.4} & \heatcell{31.3}{10.4}{39.2} & \heatcell{22.1}{21.7}{69.4} & \heatcell{38.1}{10.5}{59.3} &
%   \heatcell{4.1}{0.3}{60.7} & \heatcellb{32.8}{8.2}{32.8} & \heatcell{26.7}{0.0}{55.6} &
%   \heatcell{26.7}{0.4}{49.2} & \heatcell{36.1}{12.7}{60.8} & \heatcell{16.4}{10.7}{61.3} &
%   \heatcell{41.3}{33.3}{70.4} & \heatcell{8.8}{4.2}{41.2} & \heatcell{19.1}{0.4}{30.8} \\
%   \midrule
%   \midrule
%   \rowcolor[HTML]{A6E3E9}
%   \multicolumn{17}{c}{\bfseries\itshape Medical MLLMs} \\
%   \midrule
%   Lingshu-7B~\cite{xu2025lingshu} & 7B & 64 & \heatcell{25.0}{20.1}{41.1} & \heatcell{27.6}{19.3}
%   {49.4} & \heatcell{23.6}{10.4}{39.2} & \NAcell & \heatcell{46.2}{10.5}{59.3} & \heatcell{8.1}{0.3}
%   {60.7} & \heatcell{12.9}{8.2}{32.8} & \heatcell{11.1}{0.0}{55.6} & \heatcell{19.1}{0.4}{49.2} &
%   \heatcell{25.5}{12.7}{60.8} & \heatcell{33.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} &
%   \heatcell{20.8}{4.2}{41.2} & \heatcell{2.9}{0.4}{30.8} \\
%   Lingshu-32B~\cite{xu2025lingshu} & 32B & 64 & \heatcell{27.9}{20.1}{41.1} & \heatcell{25.1}{19.3}
%   {49.4} & \heatcell{33.3}{10.4}{39.2} & \heatcell{38.6}{21.7}{69.4} & \heatcell{35.9}{10.5}{59.3} &
%   \heatcell{12.8}{0.3}{60.7} & \heatcell{31.9}{8.2}{32.8} & \heatcell{31.9}{0.0}{55.6} &
%   \heatcell{17.0}{0.4}{49.2} & \heatcell{30.6}{12.7}{60.8} & \heatcell{50.0}{10.7}{61.3} &
%   \heatcell{34.6}{33.3}{70.4} & \heatcell{16.7}{4.2}{41.2} & \NAcell \\
%   Hulu-Med-7B~\cite{hulumed} & 7B & 32 & \heatcell{26.2}{20.1}{41.1} & \heatcell{27.3}{19.3}{49.4} &
%   \heatcell{17.3}{10.4}{39.2} & \NAcell & \heatcell{38.5}{10.5}{59.3} & \heatcell{21.6}{0.3}{60.7} &
%   \heatcell{25.9}{8.2}{32.8} & \heatcellb{55.6}{0.0}{55.6} & \heatcell{25.5}{0.4}{49.2} &
%   \heatcell{24.4}{12.7}{60.8} & \heatcell{31.4}{10.7}{61.3} & \heatcell{33.3}{33.3}{70.4} &
%   \heatcell{25.0}{4.2}{41.2} & \heatcell{26.5}{0.4}{30.8} \\
%   HuatuoGPT-Vision-7B~\cite{huatuogptvision} & 7B & 64 & \heatcell{20.1}{20.1}{41.1} &
%   \heatcell{21.7}{19.3}{49.4} & \heatcell{23.6}{10.4}{39.2} & \NAcell & \heatcell{53.8}{10.5}{59.3}
%   & \heatcell{8.1}{0.3}{60.7} & \heatcell{8.2}{8.2}{32.8} & \heatcell{0.0}{0.0}{55.6} &
%   \heatcell{34.0}{0.4}{49.2} & \heatcell{12.7}{12.7}{60.8} & \heatcell{29.4}{10.7}{61.3} &
%   \heatcell{33.3}{33.3}{70.4} & \heatcell{20.8}{4.2}{41.2} & \heatcell{14.7}{0.4}{30.8} \\
%   \bottomrule
%   \end{tabular}
%   \end{adjustbox}
%   \end{table*}


% \begin{table*}[ht]
% \renewcommand{\arraystretch}{1.18}
% \centering
% \caption{Main results on MLVBench. Size denotes model parameters and $F$ the frame budget. The first row is a prompt-only Qwen3-VL-8B sanity check for text shortcuts. Best results are in \textbf{bold}. Darker shades indicate stronger values within each column.}
% \label{tab:main_results}
% \begin{adjustbox}{width=1\linewidth}
% \scriptsize
% \setlength{\tabcolsep}{2.7pt}
% \begin{tabular}{l c c c c c c c c c c c c c c c c}
% \toprule
% \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{F}} & \multirow{2}{*}{\textbf{Ov.}} & \multicolumn{8}{c}{\textbf{Fine-grained Understanding}} & \multicolumn{5}{c}{\textbf{Semantic Reasoning}} \\
% \cmidrule(lr){5-12}\cmidrule(lr){13-17}
%  &  &  &  & PR & SD & RL & BPQ & LLS & Site & Hist & Size & IR & WR & RSR & CPR & LD \\
% \midrule
% Text-only & 8B & 0 & \heatcell{27.8}{20.1}{41.1} & \heatcell{26.8}{19.3}{49.4} & \heatcell{32.5}{10.4}{39.2} & \heatcell{46.7}{20.9}{69.4} & \heatcell{41.0}{10.5}{59.3} & \heatcell{0.0}{0.0}{60.7} & \heatcell{23.4}{8.2}{32.8} & \heatcell{14.9}{0.0}{55.6} & \heatcell{2.1}{0.4}{49.2} & \heatcell{34.5}{12.7}{60.8} & \heatcell{26.9}{10.7}{61.3} & \heatcell{38.5}{33.3}{70.4} & \heatcell{11.5}{4.2}{41.2} & \heatcell{21.9}{0.4}{37.6} \\
% \midrule
% \midrule
% \rowcolor[HTML]{E3FDFD}
% \multicolumn{17}{c}{\bfseries\itshape Closed-Source MLLMs} \\
% \midrule
% GPT-5.4-mini~\protect\cite{gpt54mini} & -- & 32 & \heatcell{31.2}{20.1}{41.1} & \heatcellb{49.4}{19.3}{49.4} & \heatcell{20.6}{10.4}{39.2} & \heatcell{59.3}{20.9}{69.4} & \heatcell{40.8}{10.5}{59.3} & \heatcell{0.5}{0.0}{60.7} & \heatcell{19.4}{8.2}{32.8} & \heatcell{20.7}{0.0}{55.6} & \heatcell{19.3}{0.4}{49.2} & \heatcell{40.6}{12.7}{60.8} & \heatcell{41.2}{10.7}{61.3} & \heatcell{59.1}{33.3}{70.4} & \heatcell{10.8}{4.2}{41.2} & \heatcell{19.5}{0.4}{37.6} \\
% GPT-5.4~\protect\cite{gpt54} & -- & 32 & \heatcell{32.6}{20.1}{41.1} & \heatcell{30.8}{19.3}{49.4} & \heatcell{19.2}{10.4}{39.2} & \heatcell{60.7}{20.9}{69.4} & \heatcell{39.4}{10.5}{59.3} & \heatcell{20.6}{0.0}{60.7} & \heatcell{29.3}{8.2}{32.8} & \heatcell{20.5}{0.0}{55.6} & \heatcell{30.8}{0.4}{49.2} & \heatcell{20.7}{12.7}{60.8} & \heatcell{39.2}{10.7}{61.3} & \heatcell{69.4}{33.3}{70.4} & \heatcell{30.5}{4.2}{41.2} & \heatcell{19.2}{0.4}{37.6} \\
% Gemini-3.1-Pro-Preview~\protect\cite{gemini3propreview} & -- & 32 & \heatcellb{41.1}{20.1}{41.1} & \heatcell{29.4}{19.3}{49.4} & \heatcell{30.6}{10.4}{39.2} & \heatcell{39.2}{20.9}{69.4} & \heatcellb{59.3}{10.5}{59.3} & \heatcellb{60.7}{0.0}{60.7} & \heatcell{20.5}{8.2}{32.8} & \heatcell{30.9}{0.0}{55.6} & \heatcellb{49.2}{0.4}{49.2} & \heatcellb{60.8}{12.7}{60.8} & \heatcellb{61.3}{10.7}{61.3} & \heatcell{69.1}{33.3}{70.4} & \heatcell{30.6}{4.2}{41.2} & \heatcell{0.4}{0.4}{37.6} \\
% Gemini-2.5-Flash~\protect\cite{gemini25flash} & -- & 32 & \heatcell{27.4}{20.1}{41.1} & \heatcell{19.3}{19.3}{49.4} & \heatcell{30.5}{10.4}{39.2} & \heatcellb{69.4}{20.9}{69.4} & \heatcell{20.7}{10.5}{59.3} & \heatcell{0.3}{0.0}{60.7} & \heatcell{31.2}{8.2}{32.8} & \heatcell{9.4}{0.0}{55.6} & \heatcell{0.6}{0.4}{49.2} & \heatcell{50.8}{12.7}{60.8} & \heatcell{10.7}{10.7}{61.3} & \heatcell{39.2}{33.3}{70.4} & \heatcell{40.6}{4.2}{41.2} & \heatcell{30.8}{0.4}{37.6} \\
% Kimi-K2.5~\protect\cite{kimi25} & -- & 64 & \heatcell{29.3}{20.1}{41.1} & \heatcell{30.5}{19.3}{49.4} & \heatcell{19.5}{10.4}{39.2} & \heatcell{50.8}{20.9}{69.4} & \heatcell{39.2}{10.5}{59.3} & \heatcell{10.7}{0.0}{60.7} & \heatcell{10.4}{8.2}{32.8} & \heatcell{9.3}{0.0}{55.6} & \heatcell{20.6}{0.4}{49.2} & \heatcell{59.1}{12.7}{60.8} & \heatcell{30.8}{10.7}{61.3} & \heatcell{50.5}{33.3}{70.4} & \heatcellb{41.2}{4.2}{41.2} & \heatcell{20.7}{0.4}{37.6} \\
% Qwen3.5-Plus~\protect\cite{qwen35suite} & -- & 64 & \heatcell{28.1}{20.1}{41.1} & \heatcell{49.2}{19.3}{49.4} & \heatcell{10.4}{10.4}{39.2} & \heatcell{60.8}{20.9}{69.4} & \heatcell{10.7}{10.5}{59.3} & \heatcell{30.6}{0.0}{60.7} & \heatcell{10.5}{8.2}{32.8} & \heatcell{0.3}{0.0}{55.6} & \heatcell{20.4}{0.4}{49.2} & \heatcell{20.5}{12.7}{60.8} & \heatcell{29.3}{10.7}{61.3} & \heatcellb{70.4}{33.3}{70.4} & \heatcell{30.8}{4.2}{41.2} & \heatcell{19.3}{0.4}{37.6} \\
% Qwen3.6-Plus~\protect\cite{qwen36plus} & -- & 64 & \heatcell{25.8}{20.1}{41.1} & \heatcell{20.6}{19.3}{49.4} & \heatcellb{39.2}{10.4}{39.2} & \heatcell{50.5}{20.9}{69.4} & \heatcell{10.5}{10.5}{59.3} & \heatcell{20.4}{0.0}{60.7} & \heatcell{9.3}{8.2}{32.8} & \heatcell{20.7}{0.0}{55.6} & \heatcell{30.8}{0.4}{49.2} & \heatcell{19.4}{12.7}{60.8} & \heatcell{20.5}{10.7}{61.3} & \heatcell{59.1}{33.3}{70.4} & \heatcell{40.6}{4.2}{41.2} & \heatcell{0.5}{0.4}{37.6} \\
% Qwen3.5-Flash~\protect\cite{qwen35suite} & -- & 64 & \heatcell{25.9}{20.1}{41.1} & \heatcell{19.4}{19.3}{49.4} & \heatcell{10.7}{10.4}{39.2} & \heatcell{39.3}{20.9}{69.4} & \heatcell{30.8}{10.5}{59.3} & \heatcell{19.4}{0.0}{60.7} & \heatcell{10.3}{8.2}{32.8} & \heatcell{10.5}{0.0}{55.6} & \heatcell{0.4}{0.4}{49.2} & \heatcell{39.2}{12.7}{60.8} & \heatcell{30.6}{10.7}{61.3} & \heatcell{59.3}{33.3}{70.4} & \heatcell{30.5}{4.2}{41.2} & \heatcell{29.3}{0.4}{37.6} \\
% \midrule
% \rowcolor[HTML]{CBF1F5}
% \multicolumn{17}{c}{\bfseries\itshape Open-Source MLLMs} \\
% \midrule
% Qwen3-VL-4B~\protect\cite{qwen3vl} & 4B & 64 & \heatcell{23.1}{20.1}{41.1} & \heatcell{22.0}{19.3}{49.4} & \heatcell{35.5}{10.4}{39.2} & \heatcell{20.9}{20.9}{69.4} & \heatcell{28.2}{10.5}{59.3} & \heatcell{5.4}{0.0}{60.7} & \heatcell{11.8}{8.2}{32.8} & \heatcell{11.1}{0.0}{55.6} & \heatcell{23.4}{0.4}{49.2} & \heatcell{22.5}{12.7}{60.8} & \heatcell{39.2}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} & \heatcell{12.5}{4.2}{41.2} & \heatcell{29.4}{0.4}{37.6} \\
% MiniCPM-V 2.6~\protect\cite{minicpmv26} & 8B & 64 & \heatcell{23.1}{20.1}{41.1} & \heatcell{26.5}{19.3}{49.4} & \heatcell{17.3}{10.4}{39.2} & \heatcell{26.4}{20.9}{69.4} & \heatcell{28.2}{10.5}{59.3} & \heatcell{5.4}{0.0}{60.7} & \heatcell{17.6}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{25.5}{0.4}{49.2} & \heatcell{19.3}{12.7}{60.8} & \heatcell{41.2}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} & \heatcell{20.8}{4.2}{41.2} & \heatcell{5.9}{0.4}{37.6} \\
% Qwen3-VL-8B~\protect\cite{qwen3vl} & 8B & 64 & \heatcell{26.2}{20.1}{41.1} & \heatcell{24.9}{19.3}{49.4} & \heatcell{30.9}{10.4}{39.2} & \heatcell{25.2}{20.9}{69.4} & \heatcell{35.9}{10.5}{59.3} & \heatcell{5.4}{0.0}{60.7} & \heatcell{24.7}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{21.3}{0.4}{49.2} & \heatcell{29.8}{12.7}{60.8} & \heatcell{35.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} & \heatcell{4.2}{4.2}{41.2} & \heatcell{20.6}{0.4}{37.6} \\
% InternVL3.5-8B~\protect\cite{internvl3.5} & 8B & 64 & \heatcell{27.0}{20.1}{41.1} & \heatcell{25.8}{19.3}{49.4} & \heatcell{30.0}{10.4}{39.2} & \heatcell{24.8}{20.9}{69.4} & \heatcell{38.5}{10.5}{59.3} & \heatcell{13.5}{0.0}{60.7} & \heatcell{17.6}{8.2}{32.8} & \heatcell{33.3}{0.0}{55.6} & \heatcell{17.0}{0.4}{49.2} & \heatcell{30.9}{12.7}{60.8} & \heatcell{37.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} & \heatcell{20.8}{4.2}{41.2} & \heatcell{29.4}{0.4}{37.6} \\
% LLaVA-Video-7B~\protect\cite{zhang2024llavanextvideo} & 7B & 64 & \heatcell{24.9}{20.1}{41.1} & \heatcell{23.2}{19.3}{49.4} & \heatcell{27.6}{10.4}{39.2} & \heatcell{46.4}{20.9}{69.4} & \heatcell{37.6}{10.5}{59.3} & \heatcell{0.0}{0.0}{60.7} & \heatcell{15.5}{8.2}{32.8} & \heatcell{17.7}{0.0}{55.6} & \heatcell{2.2}{0.4}{49.2} & \heatcell{31.1}{12.3}{60.8} & \heatcell{26.3}{10.7}{61.3} & \heatcell{49.3}{19.2}{70.4} & \heatcell{12.2}{4.2}{41.2} & \heatcell{16.0}{0.4}{37.6} \\
% LLaVA-Video-72B~\protect\cite{zhang2024llavanextvideo} & 72B & 64 & \heatcell{29.4}{20.1}{41.1} & \heatcell{27.7}{19.3}{49.4} & \heatcell{32.1}{10.4}{39.2} & \heatcell{50.9}{20.9}{69.4} & \heatcell{42.1}{10.5}{59.3} & \heatcell{2.6}{0.0}{60.7} & \heatcell{20.0}{8.2}{32.8} & \heatcell{22.2}{0.0}{55.6} & \heatcell{6.7}{0.4}{49.2} & \heatcell{35.6}{12.7}{60.8} & \heatcell{30.8}{10.7}{61.3} & \heatcell{53.8}{33.3}{70.4} & \heatcell{16.7}{4.2}{41.2} & \heatcell{20.5}{0.4}{37.6} \\
% AKS~\protect\cite{AKS} & 8B & 128 & \heatcell{27.3}{20.1}{41.1} & \heatcell{25.0}{19.3}{49.4} & \heatcell{31.2}{10.4}{39.2} & \heatcell{30.0}{20.9}{69.4} & \heatcell{35.9}{10.5}{59.3} & \heatcell{2.6}{0.0}{60.7} & \heatcell{29.8}{8.2}{32.8} & \heatcell{23.4}{0.0}{55.6} & \heatcell{31.9}{0.4}{49.2} & \heatcell{34.0}{12.7}{60.8} & \heatcell{15.4}{10.7}{61.3} & \heatcell{50.0}{33.3}{70.4} & \heatcell{7.7}{4.2}{41.2} & \heatcell{18.8}{0.4}{37.6} \\
% ViLAMP~\protect\cite{vilamp} & 8B & 128 & \heatcell{27.0}{20.1}{41.1} & \heatcell{24.8}{19.3}{49.4} & \heatcell{30.4}{10.4}{39.2} & \heatcell{21.7}{20.9}{69.4} & \heatcell{38.5}{10.5}{59.3} & \heatcell{5.1}{0.0}{60.7} & \heatcell{31.9}{8.2}{32.8} & \heatcell{25.5}{0.0}{55.6} & \heatcell{27.7}{0.4}{49.2} & \heatcell{35.3}{12.7}{60.8} & \heatcell{15.4}{10.7}{61.3} & \heatcell{42.3}{33.3}{70.4} & \heatcell{7.7}{4.2}{41.2} & \heatcell{18.8}{0.4}{37.6} \\
% WFS-SB~\protect\cite{chen2026wavelet} & 8B & 128 & \heatcell{28.1}{20.1}{41.1} & \heatcell{25.1}{19.3}{49.4} & \heatcell{31.3}{10.4}{39.2} & \heatcell{22.1}{20.9}{69.4} & \heatcell{38.1}{10.5}{59.3} & \heatcell{4.1}{0.0}{60.7} & \heatcellb{32.8}{8.2}{32.8} & \heatcell{26.7}{0.0}{55.6} & \heatcell{26.7}{0.4}{49.2} & \heatcell{36.1}{12.7}{60.8} & \heatcell{16.4}{10.7}{61.3} & \heatcell{41.3}{33.3}{70.4} & \heatcell{8.8}{4.2}{41.2} & \heatcell{19.1}{0.4}{37.6} \\
% \midrule
% \rowcolor[HTML]{A6E3E9}
% \multicolumn{17}{c}{\bfseries\itshape Medical MLLMs} \\
% \midrule
% Lingshu-7B~\protect\cite{xu2025lingshu} & 7B & 64 & \heatcell{25.0}{20.1}{41.1} & \heatcell{27.6}{19.3}{49.4} & \heatcell{23.6}{10.4}{39.2} & \heatcell{28.2}{20.9}{69.4} & \heatcell{46.2}{10.5}{59.3} & \heatcell{8.1}{0.0}{60.7} & \heatcell{12.9}{8.2}{32.8} & \heatcell{11.1}{0.0}{55.6} & \heatcell{19.1}{0.4}{49.2} & \heatcell{25.5}{12.7}{60.8} & \heatcell{33.3}{10.7}{61.3} & \heatcell{66.7}{33.3}{70.4} & \heatcell{20.8}{4.2}{41.2} & \heatcell{2.9}{0.4}{37.6} \\
% Lingshu-32B~\protect\cite{xu2025lingshu} & 32B & 64 & \heatcell{27.9}{20.1}{41.1} & \heatcell{25.1}{19.3}{49.4} & \heatcell{33.3}{10.4}{39.2} & \heatcell{38.6}{20.9}{69.4} & \heatcell{35.9}{10.5}{59.3} & \heatcell{12.8}{0.0}{60.7} & \heatcell{31.9}{8.2}{32.8} & \heatcell{31.9}{0.0}{55.6} & \heatcell{17.0}{0.4}{49.2} & \heatcell{30.6}{12.7}{60.8} & \heatcell{50.0}{10.7}{61.3} & \heatcell{34.6}{33.3}{70.4} & \heatcell{16.7}{4.2}{41.2} & \heatcellb{37.6}{0.4}{37.6} \\
% Hulu-Med-7B~\protect\cite{hulumed} & 7B & 32 & \heatcell{26.2}{20.1}{41.1} & \heatcell{27.3}{19.3}{49.4} & \heatcell{17.3}{10.4}{39.2} & \heatcell{27.6}{20.9}{69.4} & \heatcell{38.5}{10.5}{59.3} & \heatcell{21.6}{0.0}{60.7} & \heatcell{25.9}{8.2}{32.8} & \heatcellb{55.6}{0.0}{55.6} & \heatcell{25.5}{0.4}{49.2} & \heatcell{24.4}{12.7}{60.8} & \heatcell{31.4}{10.7}{61.3} & \heatcell{33.3}{33.3}{70.4} & \heatcell{25.0}{4.2}{41.2} & \heatcell{26.5}{0.4}{37.6} \\
% HuatuoGPT-Vision-7B~\protect\cite{huatuogptvision} & 7B & 64 & \heatcell{20.1}{20.1}{41.1} & \heatcell{21.7}{19.3}{49.4} & \heatcell{23.6}{10.4}{39.2} & \heatcell{21.6}{20.9}{69.4} & \heatcell{53.8}{10.5}{59.3} & \heatcell{8.1}{0.0}{60.7} & \heatcell{8.2}{8.2}{32.8} & \heatcell{0.0}{0.0}{55.6} & \heatcell{34.0}{0.4}{49.2} & \heatcell{12.7}{12.7}{60.8} & \heatcell{29.4}{10.7}{61.3} & \heatcell{33.3}{33.3}{70.4} & \heatcell{20.8}{4.2}{41.2} & \heatcell{14.7}{0.4}{37.6} \\
% MedGRPO~\protect\cite{medgrpo} & 7B & 64 & \heatcell{20.1}{20.1}{41.1} & \heatcell{22.1}{19.3}{49.4} & \heatcell{19.6}{10.4}{39.2} & \heatcell{23.3}{20.9}{69.4} & \heatcell{35.9}{10.5}{59.3} & \heatcell{12.8}{0.0}{60.7} & \heatcell{19.1}{8.2}{32.8} & \heatcell{8.5}{0.0}{55.6} & \heatcell{48.9}{0.4}{49.2} & \heatcell{12.3}{12.3}{60.8} & \heatcell{26.9}{10.7}{61.3} & \heatcell{19.2}{19.2}{70.4} & \heatcell{11.5}{4.2}{41.2} & \heatcell{9.4}{0.4}{37.6} \\

% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % \vspace{-4mm}
% \end{table*}



\begin{table*}[ht]
\renewcommand{\arraystretch}{1.18}
\centering
\caption{Main results on \ours. Input reports the visual input protocol: a number indicates a fixed uniform sampled frame budget, while ``1 FPS'' indicates fps-based video sampling. Best results are in \textbf{bold}. Darker shades indicate stronger values within each column.}
\label{tab:main_results}
\begin{adjustbox}{width=1\linewidth}
\scriptsize
\setlength{\tabcolsep}{2.7pt}
\begin{tabular}{l c c c c c c c c c c c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Input}} & \multirow{2}{*}{\textbf{Ov.}} & \multicolumn{8}{c}{\textbf{Fine-grained Understanding}} & \multicolumn{5}{c}{\textbf{Semantic Reasoning}} \\
\cmidrule(lr){5-12}\cmidrule(lr){13-17}
 &  &  &  & PR & SD & RL & BPQ & LLS & Site & Hist & Size & IR & WR & RSR & CPR & LA \\

\midrule
% \multicolumn{3}{l}{\itshape Question count} & \makebox[2.2em][r]{1253} & \makebox[2.2em][r]{517} & \makebox[2.2em][r]{112} & \makebox[2.2em][r]{60} & \makebox[2.2em][r]{39} & \makebox[2.2em][r]{39} & \makebox[2.2em][r]{47} & \makebox[2.2em][r]{47} & \makebox[2.2em][r]{47} & \makebox[2.2em][r]{235} & \makebox[2.2em][r]{26} & \makebox[2.2em][r]{26} & \makebox[2.2em][r]{26} & \makebox[2.2em][r]{32} \\
\midrule
\rowcolor[HTML]{E3FDFD}
\multicolumn{17}{c}{\bfseries\itshape Closed-Source MLLMs} \\
\midrule
GPT-5.4-mini~\protect\cite{gpt54mini} & -- & 1 FPS & \heatcell{31.2}{18.2}{41.1} & \heatcell{35.0}{17.0}{38.9} & \heatcell{17.0}{8.0}{40.2} & \heatcell{58.3}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{0.0}{0.0}{61.5} & \heatcell{17.0}{8.5}{31.9} & \heatcell{19.1}{0.0}{55.3} & \heatcell{17.0}{0.0}{48.9} & \heatcell{34.5}{12.3}{62.6} & \heatcell{42.3}{11.5}{61.5} & \heatcell{57.7}{19.2}{69.2} & \heatcell{11.5}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
GPT-5.4~\protect\cite{gpt54} & -- & 1 FPS & \heatcell{32.6}{18.2}{41.1} & \heatcell{36.4}{17.0}{38.9} & \heatcell{20.5}{8.0}{40.2} & \heatcell{61.7}{11.7}{70.0} & \heatcell{41.0}{10.3}{59.0} & \heatcell{20.5}{0.0}{61.5} & \heatcell{29.8}{8.5}{31.9} & \heatcell{21.3}{0.0}{55.3} & \heatcell{31.9}{0.0}{48.9} & \heatcell{23.4}{12.3}{62.6} & \heatcell{38.5}{11.5}{61.5} & \heatcellb{69.2}{19.2}{69.2} & \heatcell{30.8}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
Gemini-3.1-Pro-Preview~\protect\cite{gemini3propreview} & -- & 1 FPS & \heatcellb{41.1}{18.2}{41.1} & \heatcell{33.3}{17.0}{38.9} & \heatcell{31.2}{8.0}{40.2} & \heatcell{40.0}{11.7}{70.0} & \heatcellb{59.0}{10.3}{59.0} & \heatcellb{61.5}{0.0}{61.5} & \heatcell{21.3}{8.5}{31.9} & \heatcell{31.9}{0.0}{55.3} & \heatcellb{48.9}{0.0}{48.9} & \heatcellb{62.6}{12.3}{62.6} & \heatcellb{61.5}{11.5}{61.5} & \heatcellb{69.2}{19.2}{69.2} & \heatcell{30.8}{3.8}{42.3} & \heatcell{0.0}{0.0}{37.5} \\
Gemini-2.5-Flash~\protect\cite{gemini25flash} & -- & 1 FPS & \heatcell{27.4}{18.2}{41.1} & \heatcell{17.2}{17.0}{38.9} & \heatcell{30.4}{8.0}{40.2} & \heatcellb{70.0}{11.7}{70.0} & \heatcell{20.5}{10.3}{59.0} & \heatcell{0.0}{0.0}{61.5} & \heatcellb{31.9}{8.5}{31.9} & \heatcell{8.5}{0.0}{55.3} & \heatcell{0.0}{0.0}{48.9} & \heatcell{49.8}{12.3}{62.6} & \heatcell{11.5}{11.5}{61.5} & \heatcell{38.5}{19.2}{69.2} & \heatcellb{42.3}{3.8}{42.3} & \heatcell{31.2}{0.0}{37.5} \\
Kimi-K2.5~\protect\cite{kimi25} & -- & 1 FPS & \heatcell{29.3}{18.2}{41.1} & \heatcell{21.9}{17.0}{38.9} & \heatcell{17.9}{8.0}{40.2} & \heatcell{50.0}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{10.3}{0.0}{61.5} & \heatcell{10.6}{8.5}{31.9} & \heatcell{8.5}{0.0}{55.3} & \heatcell{19.1}{0.0}{48.9} & \heatcell{54.9}{12.3}{62.6} & \heatcell{30.8}{11.5}{61.5} & \heatcell{50.0}{19.2}{69.2} & \heatcellb{42.3}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
Qwen3.5-Plus~\protect\cite{qwen35suite} & -- & 1 FPS & \heatcell{28.1}{18.2}{41.1} & \heatcellb{38.9}{17.0}{38.9} & \heatcell{8.0}{8.0}{40.2} & \heatcell{60.0}{11.7}{70.0} & \heatcell{10.3}{10.3}{59.0} & \heatcell{30.8}{0.0}{61.5} & \heatcell{8.5}{8.5}{31.9} & \heatcell{0.0}{0.0}{55.3} & \heatcell{19.1}{0.0}{48.9} & \heatcell{16.2}{12.3}{62.6} & \heatcell{26.9}{11.5}{61.5} & \heatcellb{69.2}{19.2}{69.2} & \heatcell{30.8}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
Qwen3.6-Plus~\protect\cite{qwen36plus} & -- & 1 FPS & \heatcell{25.8}{18.2}{41.1} & \heatcell{24.0}{17.0}{38.9} & \heatcellb{40.2}{8.0}{40.2} & \heatcell{51.7}{11.7}{70.0} & \heatcell{10.3}{10.3}{59.0} & \heatcell{20.5}{0.0}{61.5} & \heatcell{10.6}{8.5}{31.9} & \heatcell{21.3}{0.0}{55.3} & \heatcell{31.9}{0.0}{48.9} & \heatcell{21.3}{12.3}{62.6} & \heatcell{19.2}{11.5}{61.5} & \heatcell{57.7}{19.2}{69.2} & \heatcellb{42.3}{3.8}{42.3} & \heatcell{0.0}{0.0}{37.5} \\
Qwen3.5-Flash~\protect\cite{qwen35suite} & -- & 1 FPS & \heatcell{25.9}{18.2}{41.1} & \heatcell{23.4}{17.0}{38.9} & \heatcell{11.6}{8.0}{40.2} & \heatcell{40.0}{11.7}{70.0} & \heatcell{30.8}{10.3}{59.0} & \heatcell{20.5}{0.0}{61.5} & \heatcell{10.6}{8.5}{31.9} & \heatcell{10.6}{0.0}{55.3} & \heatcell{0.0}{0.0}{48.9} & \heatcell{41.3}{12.3}{62.6} & \heatcell{30.8}{11.5}{61.5} & \heatcell{57.7}{19.2}{69.2} & \heatcell{30.8}{3.8}{42.3} & \heatcell{28.1}{0.0}{37.5} \\
\midrule
\rowcolor[HTML]{CBF1F5}
\multicolumn{17}{c}{\bfseries\itshape Open-Source MLLMs} \\
\midrule
Qwen3-VL-4B~\protect\cite{qwen3vl} & 4B & 1~FPS & \heatcell{23.1}{18.2}{41.1} & \heatcell{21.5}{17.0}{38.9} & \heatcell{35.7}{8.0}{40.2} & \heatcell{20.0}{11.7}{70.0} & \heatcell{28.2}{10.3}{59.0} & \heatcell{5.1}{0.0}{61.5} & \heatcell{12.8}{8.5}{31.9} & \heatcell{10.6}{0.0}{55.3} & \heatcell{23.4}{0.0}{48.9} & \heatcell{22.1}{12.3}{62.6} & \heatcell{38.5}{11.5}{61.5} & \heatcell{65.4}{19.2}{69.2} & \heatcell{11.5}{3.8}{42.3} & \heatcell{28.1}{0.0}{37.5} \\
MiniCPM-V 2.6~\protect\cite{minicpmv26} & 8B & 64 & \heatcell{23.1}{18.2}{41.1} & \heatcell{24.6}{17.0}{38.9} & \heatcell{17.0}{8.0}{40.2} & \heatcell{26.7}{11.7}{70.0} & \heatcell{28.2}{10.3}{59.0} & \heatcell{5.1}{0.0}{61.5} & \heatcell{17.0}{8.5}{31.9} & \heatcell{34.0}{0.0}{55.3} & \heatcell{25.5}{0.0}{48.9} & \heatcell{18.3}{12.3}{62.6} & \heatcell{42.3}{11.5}{61.5} & \heatcell{65.4}{19.2}{69.2} & \heatcell{19.2}{3.8}{42.3} & \heatcell{6.2}{0.0}{37.5} \\
Qwen3-VL-8B~\protect\cite{qwen3vl} & 8B & 1~FPS & \heatcell{26.2}{18.2}{41.1} & \heatcell{23.6}{17.0}{38.9} & \heatcell{30.4}{8.0}{40.2} & \heatcell{25.0}{11.7}{70.0} & \heatcell{35.9}{10.3}{59.0} & \heatcell{5.1}{0.0}{61.5} & \heatcell{25.5}{8.5}{31.9} & \heatcell{34.0}{0.0}{55.3} & \heatcell{21.3}{0.0}{48.9} & \heatcell{29.4}{12.3}{62.6} & \heatcell{34.6}{11.5}{61.5} & \heatcell{65.4}{19.2}{69.2} & \heatcell{3.8}{3.8}{42.3} & \heatcell{21.9}{0.0}{37.5} \\
InternVL3.5-8B~\protect\cite{internvl3.5} & 8B & 64 & \heatcell{27.0}{18.2}{41.1} & \heatcell{24.4}{17.0}{38.9} & \heatcell{29.5}{8.0}{40.2} & \heatcell{25.0}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{12.8}{0.0}{61.5} & \heatcell{17.0}{8.5}{31.9} & \heatcell{34.0}{0.0}{55.3} & \heatcell{17.0}{0.0}{48.9} & \heatcell{30.2}{12.3}{62.6} & \heatcell{38.5}{11.5}{61.5} & \heatcell{65.4}{19.2}{69.2} & \heatcell{19.2}{3.8}{42.3} & \heatcell{28.1}{0.0}{37.5} \\
LLaVA-Video-7B~\protect\cite{zhang2024llavanextvideo} & 7B & 1~FPS & \heatcell{24.9}{18.2}{41.1} & \heatcell{23.4}{17.0}{38.9} & \heatcell{27.7}{8.0}{40.2} & \heatcell{46.7}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{0.0}{0.0}{61.5} & \heatcell{14.9}{8.5}{31.9} & \heatcell{17.0}{0.0}{55.3} & \heatcell{2.1}{0.0}{48.9} & \heatcell{31.1}{12.3}{62.6} & \heatcell{26.9}{11.5}{61.5} & \heatcell{50.0}{19.2}{69.2} & \heatcell{11.5}{3.8}{42.3} & \heatcell{15.6}{0.0}{37.5} \\
LLaVA-Video-72B~\protect\cite{zhang2024llavanextvideo} & 72B & 1~FPS & \heatcell{29.4}{18.2}{41.1} & \heatcell{28.0}{17.0}{38.9} & \heatcell{32.1}{8.0}{40.2} & \heatcell{51.7}{11.7}{70.0} & \heatcell{41.0}{10.3}{59.0} & \heatcell{2.6}{0.0}{61.5} & \heatcell{19.1}{8.5}{31.9} & \heatcell{21.3}{0.0}{55.3} & \heatcell{6.4}{0.0}{48.9} & \heatcell{35.7}{12.3}{62.6} & \heatcell{30.8}{11.5}{61.5} & \heatcell{53.8}{19.2}{69.2} & \heatcell{15.4}{3.8}{42.3} & \heatcell{21.9}{0.0}{37.5} \\

\midrule
\rowcolor[HTML]{B9E5E8}
\multicolumn{17}{c}{\bfseries\itshape Specialized long-video methods} \\
% \addlinespace[0.1em]
\midrule
AKS~\protect\cite{AKS} & 8B & 128 & \heatcell{27.3}{18.2}{41.1} & \heatcell{25.0}{17.0}{38.9} & \heatcell{31.2}{8.0}{40.2} & \heatcell{30.0}{11.7}{70.0} & \heatcell{35.9}{10.3}{59.0} & \heatcell{2.6}{0.0}{61.5} & \heatcell{29.8}{8.5}{31.9} & \heatcell{23.4}{0.0}{55.3} & \heatcell{31.9}{0.0}{48.9} & \heatcell{34.0}{12.3}{62.6} & \heatcell{15.4}{11.5}{61.5} & \heatcell{50.0}{19.2}{69.2} & \heatcell{7.7}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
ViLAMP~\protect\cite{vilamp} & 8B & 128 & \heatcell{27.0}{18.2}{41.1} & \heatcell{24.8}{17.0}{38.9} & \heatcell{30.4}{8.0}{40.2} & \heatcell{21.7}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{5.1}{0.0}{61.5} & \heatcellb{31.9}{8.5}{31.9} & \heatcell{25.5}{0.0}{55.3} & \heatcell{27.7}{0.0}{48.9} & \heatcell{35.3}{12.3}{62.6} & \heatcell{15.4}{11.5}{61.5} & \heatcell{42.3}{19.2}{69.2} & \heatcell{7.7}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
WFS-SB~\protect\cite{chen2026wavelet} & 8B & 128 & \heatcell{28.1}{18.2}{41.1} & \heatcell{26.5}{17.0}{38.9} & \heatcell{31.2}{8.0}{40.2} & \heatcell{21.7}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{5.1}{0.0}{61.5} & \heatcellb{31.9}{8.5}{31.9} & \heatcell{27.7}{0.0}{55.3} & \heatcell{27.7}{0.0}{48.9} & \heatcell{36.6}{12.3}{62.6} & \heatcell{15.4}{11.5}{61.5} & \heatcell{42.3}{19.2}{69.2} & \heatcell{7.7}{3.8}{42.3} & \heatcell{18.8}{0.0}{37.5} \\
VideoLLaMA3-7B~\protect\cite{damonlpsg2025videollama3} & 7B & 1~FPS & \heatcell{22.7}{18.2}{41.1} & \heatcell{25.1}{17.0}{38.9} & \heatcell{18.8}{8.0}{40.2} & \heatcell{36.7}{11.7}{70.0} & \heatcell{20.5}{10.3}{59.0} & \heatcell{7.7}{0.0}{61.5} & \heatcell{29.8}{8.5}{31.9} & \heatcell{8.5}{0.0}{55.3} & \heatcell{10.6}{0.0}{48.9} & \heatcell{22.6}{12.3}{62.6} & \heatcell{15.4}{11.5}{61.5} & \heatcell{26.9}{19.2}{69.2} & \heatcell{7.7}{3.8}{42.3} & \heatcell{34.4}{0.0}{37.5} \\
LongVA-7B-DPO~\protect\cite{zhang2024longva} & 7B & 512 & \heatcell{18.2}{18.2}{41.1} & \heatcell{17.0}{17.0}{38.9} & \heatcell{20.5}{8.0}{40.2} & \heatcell{15.0}{11.7}{70.0} & \heatcell{33.3}{10.3}{59.0} & \heatcell{33.3}{0.0}{61.5} & \heatcell{21.3}{8.5}{31.9} & \heatcell{21.3}{0.0}{55.3} & \heatcell{14.9}{0.0}{48.9} & \heatcell{16.2}{12.3}{62.6} & \heatcell{23.1}{11.5}{61.5} & \heatcell{19.2}{19.2}{69.2} & \heatcell{3.8}{3.8}{42.3} & \heatcell{15.6}{0.0}{37.5} \\
VideoChat-Flash-7B~\protect\cite{li2024videochatflash} & 7B & 1~FPS & \heatcell{24.9}{18.2}{41.1} & \heatcell{25.1}{17.0}{38.9} & \heatcell{30.4}{8.0}{40.2} & \heatcell{11.7}{11.7}{70.0} & \heatcell{33.3}{10.3}{59.0} & \heatcell{0.0}{0.0}{61.5} & \heatcell{23.4}{8.5}{31.9} & \heatcell{10.6}{0.0}{55.3} & \heatcell{19.1}{0.0}{48.9} & \heatcell{31.1}{12.3}{62.6} & \heatcell{19.2}{11.5}{61.5} & \heatcell{61.5}{19.2}{69.2} & \heatcell{7.7}{3.8}{42.3} & \heatcell{21.9}{0.0}{37.5} \\
\midrule
\rowcolor[HTML]{A6E3E9}
\multicolumn{17}{c}{\bfseries\itshape Medical MLLMs} \\
\midrule
Lingshu-7B~\protect\cite{xu2025lingshu} & 7B & 1~FPS & \heatcell{25.0}{18.2}{41.1} & \heatcell{26.7}{17.0}{38.9} & \heatcell{23.2}{8.0}{40.2} & \heatcell{28.3}{11.7}{70.0} & \heatcell{46.2}{10.3}{59.0} & \heatcell{7.7}{0.0}{61.5} & \heatcell{12.8}{8.5}{31.9} & \heatcell{10.6}{0.0}{55.3} & \heatcell{19.1}{0.0}{48.9} & \heatcell{25.1}{12.3}{62.6} & \heatcell{34.6}{11.5}{61.5} & \heatcell{65.4}{19.2}{69.2} & \heatcell{19.2}{3.8}{42.3} & \heatcell{3.1}{0.0}{37.5} \\
Lingshu-32B~\protect\cite{xu2025lingshu} & 32B & 1~FPS & \heatcell{27.9}{18.2}{41.1} & \heatcell{24.0}{17.0}{38.9} & \heatcell{33.0}{8.0}{40.2} & \heatcell{38.3}{11.7}{70.0} & \heatcell{35.9}{10.3}{59.0} & \heatcell{12.8}{0.0}{61.5} & \heatcellb{31.9}{8.5}{31.9} & \heatcell{31.9}{0.0}{55.3} & \heatcell{17.0}{0.0}{48.9} & \heatcell{30.2}{12.3}{62.6} & \heatcell{50.0}{11.5}{61.5} & \heatcell{34.6}{19.2}{69.2} & \heatcell{15.4}{3.8}{42.3} & \heatcellb{37.5}{0.0}{37.5} \\
Hulu-Med-7B~\protect\cite{hulumed} & 7B & 1~FPS & \heatcell{26.2}{18.2}{41.1} & \heatcell{25.7}{17.0}{38.9} & \heatcell{17.0}{8.0}{40.2} & \heatcell{26.7}{11.7}{70.0} & \heatcell{38.5}{10.3}{59.0} & \heatcell{20.5}{0.0}{61.5} & \heatcell{25.5}{8.5}{31.9} & \heatcellb{55.3}{0.0}{55.3} & \heatcell{25.5}{0.0}{48.9} & \heatcell{23.8}{12.3}{62.6} & \heatcell{30.8}{11.5}{61.5} & \heatcell{34.6}{19.2}{69.2} & \heatcell{23.1}{3.8}{42.3} & \heatcell{25.0}{0.0}{37.5} \\
HuatuoGPT-Vision-7B~\protect\cite{huatuogptvision} & 7B & 1~FPS & \heatcell{20.1}{18.2}{41.1} & \heatcell{21.7}{17.0}{38.9} & \heatcell{23.2}{8.0}{40.2} & \heatcell{21.7}{11.7}{70.0} & \heatcell{53.8}{10.3}{59.0} & \heatcell{7.7}{0.0}{61.5} & \heatcell{8.5}{8.5}{31.9} & \heatcell{0.0}{0.0}{55.3} & \heatcell{34.0}{0.0}{48.9} & \heatcell{12.8}{12.3}{62.6} & \heatcell{30.8}{11.5}{61.5} & \heatcell{34.6}{19.2}{69.2} & \heatcell{19.2}{3.8}{42.3} & \heatcell{15.6}{0.0}{37.5} \\
MedGRPO~\protect\cite{medgrpo} & 7B & 1~FPS & \heatcell{20.1}{18.2}{41.1} & \heatcell{22.1}{17.0}{38.9} & \heatcell{19.6}{8.0}{40.2} & \heatcell{23.3}{11.7}{70.0} & \heatcell{35.9}{10.3}{59.0} & \heatcell{12.8}{0.0}{61.5} & \heatcell{19.1}{8.5}{31.9} & \heatcell{8.5}{0.0}{55.3} & \heatcellb{48.9}{0.0}{48.9} & \heatcell{12.3}{12.3}{62.6} & \heatcell{26.9}{11.5}{61.5} & \heatcell{19.2}{19.2}{69.2} & \heatcell{11.5}{3.8}{42.3} & \heatcell{9.4}{0.0}{37.5} \\

\bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{1mm}

% \vspace{-4mm}
\end{table*}
    


==> MLVBench_NeurIPS2026_Overleaf/tables/recent_compare.tex <==
\begin{table}[t]
\centering
\caption{Comparison with recent medical video benchmarks. }
\label{tab:recent_compare}
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l c c c c c c c}
\toprule
Dataset & Year & Surg. & Exam. & Long-context & Extremely sparse & Multi-hop & Total(h) \\
\midrule
PitVQA~\cite{he2024pitvqa} & 2024 & \cmark & \xmark & \xmark & \xmark & \xmark & 2.1 \\
OphNet~\cite{li2024ophnet} & 2024 & \cmark & \xmark & \cmark & \xmark & \xmark & 24.5 \\
SurgeryVideoQA~\cite{thapa2025openbiomedvid} & 2025 & \cmark & \xmark & \xmark & \xmark & \xmark & 1.8 \\
MIMICEchoQA~\cite{mimicechoqa2025} & 2025 & \xmark & \cmark & \xmark & \xmark & \xmark & 5.2 \\
SurgPub-Video~\cite{surgpubvideo} & 2026 & \cmark & \xmark & \cmark & \xmark & \xmark & 31.5 \\
MedVidBench~\cite{medgrpo} & 2026 & \cmark & \cmark & \xmark & \xmark & \cmark & 22.4 \\
SUREON~\cite{qian2026sureon} & 2026 & \cmark & \xmark & \xmark & \xmark & \xmark & 3.0 \\
\midrule
\textbf{\ours (Ours)} & 2026 & \cmark & \cmark & \cmark & \cmark & \cmark & \textbf{759.0} \\
\bottomrule
\end{tabular}
}
\end{table}


==> MLVBench_NeurIPS2026_Overleaf/tables/source_datasets.tex <==
\begin{table}[t]
\centering
\caption{Source datasets used in MLVBench. We report decoded video runtime instead of JSON metadata because several raw archives preserve approximate timing fields. Task-family abbreviations follow Tab.~\ref{tab:capability_taxonomy}.}
\label{tab:source_datasets}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l l l r r r r l}
\toprule
Dataset & Organ & Scene & Videos & QA & Hours & Med. min & Task families \\
\midrule
AutoLaparo & gynecology & surgical & 20 & 44 & 22.3 & 63.0 & PR/SD/RL \\
Galar & gastrointestinal & endoscopy & 44 & 60 & 351.3 & 221.8 & PR/SD/RL \\
GraSP & urology & surgical & 13 & 112 & 32.4 & 157.4 & PR/SD/RL, IR, WR/RSR/CPR \\
MultiBypass & abdomen & surgical & 125 & 403 & 193.3 & 85.6 & PR/SD/RL \\
PitVQA & neurology & surgical & 10 & 13 & 10.5 & 63.4 & PR/SD/RL \\
REAL-Colon & gastrointestinal & colonoscopy & 39 & 251 & 17.0 & 25.3 & BPQ/LLS/LD, Site/Hist/Size \\
TMVP & cardiac & surgical & 59 & 340 & 122.7 & 118.8 & PR/SD/RL, IR \\
US-Study & obstetric/pelvic & ultrasound & 30 & 30 & 9.6 & 18.9 & PR/SD/RL \\
\midrule
Total & -- & -- & 340 & 1,253 & 759.0 & 83.2 & PR/SD/RL, IR, WR/RSR/CPR, BPQ/LLS/LD, Site/Hist/Size \\
\bottomrule
\end{tabular}
}
\end{table}



==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract, introduction, benchmark construction, and experiments all make the same core claim: existing MLLMs remain weak when sparse evidence retrieval and multi-hop reasoning must be solved jointly in full-procedure medical video.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The conclusion explicitly states two limitations of the current benchmark: reliance on public-source video diversity and a multiple-choice protocol that cannot fully capture free-form clinical reporting.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present new theoretical results or formal proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sections 3 and 4 describe the source datasets, question construction pipeline, evaluation split, task taxonomy, model families, and frame-budget settings that support the main experimental claims.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The benchmark is built on public source videos, and the benchmark assets are paired with the evaluation protocol used in this paper so the reported results can be reproduced in anonymized form.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 4 specifies the benchmark size, task structure, model categories, and frame-budget settings used in the comparisons and analyses, while Section 3 defines how the benchmark itself is constructed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: We report deterministic benchmark accuracies on a fixed evaluation set, but we do not include repeated-run error bars or formal significance tests.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper reports model types and frame budgets, but it does not provide a full per-experiment accounting of hardware, memory, runtime, and total compute.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work uses public or previously released clinical video sources for benchmark construction and is intended for evaluation research rather than direct clinical deployment, which is consistent with the NeurIPS Code of Ethics to the best of our knowledge.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: The conclusion discusses both the positive value of more realistic clinical-video evaluation and the risk of over-interpreting benchmark performance as readiness for autonomous clinical deployment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper releases an evaluation benchmark rather than a high-risk generative model, and all underlying videos come from public or previously released sources, so this question is not central to the contribution.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The source datasets and prior assets are cited throughout Sections 2 and 3, but the paper does not enumerate the full license details for every existing asset in the main text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3 documents the new benchmark through source provenance, task definitions, question construction, and evaluation protocol, and the release materials are organized to mirror that structure.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve new crowdsourcing or prospective research with human subjects; it builds a benchmark from public or previously released datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve new crowdsourcing or prospective research with human subjects, so IRB-style approval is not applicable here.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    \item[] Justification: Section 3 states that GPT-5.4 is used in the benchmark construction pipeline for question rewriting and distractor refinement, making its role explicit where it affects the released benchmark formulation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> tables/capability_taxonomy.tex <==
\begin{table}[t]
\centering
\caption{Task coverage in MLVBench. The benchmark combines fine-grained understanding over sparse evidence with multi-hop reasoning over observations scattered across full procedures.}
\label{tab:capability_taxonomy}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{3.4cm} p{8.3cm} r}
\toprule
Reasoning Focus & Representative skills & QA \\
\midrule
Fine-grained Understanding & PR/SD/RL for phase, step, region, and exam recognition; BPQ/LLS and Site/Hist/Size for quality and lesion characterization & 940 \\
Semantic Reasoning & IR for instrument recognition; WR/RSR/CPR for counting, ranking, and proportion judgment; LD for procedure-level lesion summary & 313 \\
\midrule
Total & Questions from heterogeneous long medical videos in the wild & 1,253 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/source_datasets.tex <==
\begin{table}[t]
\centering
\caption{Source datasets used in MLVBench. We report decoded video runtime instead of JSON metadata because several raw archives preserve approximate timing fields. Task-family abbreviations follow Tab.~\ref{tab:capability_taxonomy}.}
\label{tab:source_datasets}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l l l r r r r l}
\toprule
Dataset & Organ & Scene & Videos & QA & Hours & Med. min & Task families \\
\midrule
AutoLaparo & gynecology & surgical & 20 & 44 & 22.3 & 63.0 & PR/SD/RL \\
Galar & gastrointestinal & endoscopy & 44 & 60 & 351.3 & 221.8 & PR/SD/RL \\
GraSP & urology & surgical & 13 & 112 & 32.4 & 157.4 & PR/SD/RL, IR, WR/RSR/CPR \\
MultiBypass & abdomen & surgical & 125 & 403 & 193.3 & 85.6 & PR/SD/RL \\
PitVQA & neurology & surgical & 10 & 13 & 10.5 & 63.4 & PR/SD/RL \\
REAL-Colon & gastrointestinal & colonoscopy & 39 & 251 & 17.0 & 25.3 & BPQ/LLS/LD, Site/Hist/Size \\
TMVP & cardiac & surgical & 59 & 340 & 122.7 & 118.8 & PR/SD/RL, IR \\
US-Study & obstetric/pelvic & ultrasound & 30 & 30 & 9.6 & 18.9 & PR/SD/RL \\
\midrule
Total & -- & -- & 340 & 1,253 & 759.0 & 83.2 & PR/SD/RL, IR, WR/RSR/CPR, BPQ/LLS/LD, Site/Hist/Size \\
\bottomrule
\end{tabular}
}
\end{table}


